Colonel Blotto Games with Favoritism: Competitions with Pre-allocations and Asymmetric Effectiveness

We introduce the Colonel Blotto game with favoritism, an extension of the famous Colonel Blotto game where the winner-determination rule is generalized to include pre-allocations and asymmetry of the players' resources effectiveness on each battlefield. Such favoritism is found in many classical applications of the Colonel Blotto game. We focus on the Nash equilibrium. First, we consider the closely related model of all-pay auctions with favoritism and completely characterize its equilibrium. Based on this result, we prove the existence of a set of optimal univariate distributions -- which serve as candidate marginals for an equilibrium -- of the Colonel Blotto game with favoritism and show an explicit construction thereof. In several particular cases, this directly leads to an equilibrium of the Colonel Blotto game with favoritism. In other cases, we use these optimal univariate distributions to derive an approximate equilibrium with well-controlled approximation error. Finally, we propose an algorithm -- based on the notion of winding number in parametric curves -- to efficiently compute an approximation of the proposed optimal univariate distributions with arbitrarily small error.

==> EC ArXiV - Upload/Sections/abstract.tex <==
%!TEX root = ../main.tex



We introduce the \emph{Colonel Blotto game with favoritism}, an extension of the famous Colonel Blotto game where the winner-determination rule is generalized to include pre-allocations and asymmetry of the players' resources effectiveness on each battlefield. Such \emph{favoritism} is found in many classical applications of the Colonel Blotto game. We focus on the Nash equilibrium. First, we consider the closely related model of all-pay auctions with favoritism and completely characterize its equilibrium. Based on this result, we prove the existence of a set of optimal univariate distributions---which serve as candidate marginals for an equilibrium---of the Colonel Blotto game with favoritism and show an explicit construction thereof. In several particular cases, this directly leads to an equilibrium of the Colonel Blotto game with favoritism. In other cases, we use these optimal univariate distributions to derive an approximate equilibrium with well-controlled approximation error. Finally, we propose an algorithm---based on the notion of winding number in parametric curves---to efficiently compute an approximation of the proposed optimal univariate distributions with arbitrarily small error.


% Abstract by Quan before Thursday 9am
%In this work, we introduce the \emph{Colonel Blotto game with favoritism}, an extension of the famous Colonel Blotto game where the winner-determination rule is generalized to include pre-allocations and asymmetry of the players' resources effectiveness on each battlefield. Such \emph{favoritism} is found in many classical applications of the Colonel Blotto game. We focus on Nash equilibria of the Colonel Blotto game with favoritism. First, we consider and completely characterize the equilibrium of the all-pay auctions with favoritism---a game model closely related to the Colonel Blotto game. Based on this result, we prove the existence of a set of optimal univariate distributions (which serve as candidates for marginals of a possible equilibrium) of the Colonel Blotto game with favoritism and show an explicit construction thereof. From this result, we analyze several known cases of the Colonel Blotto game with favoritism where these distributions constitute an equilibrium. In other cases, based on the proposed optimal univariate distributions, we derive an approximate equilibrium with well-controlled approximation errors; we also obtain an exact equilibrium of the relaxed version where budget constraints hold in expectation (called the General Lotto game with favoritism). Finally, we propose an algorithm---based on the notion of winding numbers of parametric curves---to efficiently compute an approximation of the proposed optimal univariate distributions with arbitrarily small~errors.



% We consider the famous Colonel Blotto game, in which two players compete by allocating resources over $n$ battlefields, under a generalized winner-determination rule that includes pre-allocations and asymmetry of the player's resources effectiveness on each battlefield. Such \emph{favoritism} is found in many classical applications of the Colonel Blotto game such as political competitions, military logistics, or R\&D contests; yet it is not considered in prior works. We focus on the Nash equilibrium (NE) of the Colonel Blotto game with favoritism. We first provide a complete characterization of the NE for the related model of all-pay auctions with favoritism. Based on this result, we then prove the existence of a set of optimal univariate distributions for the Colonel Blotto game with favoritism and show an explicit construction thereof. This directly gives an NE of the CB games with favoritism under the assumption that there exists a joint distribution of these univariate distributions whose support satisfies the budget constraints. In instances where this assumption does not hold, we show that based on the proposed univariate distributions, we can obtain an approximate equilibrium with well-controlled approximation errors; moreover, we also have an exact NE of the relaxed version where budget constraints hold in expectation (the General Lotto game with favoritism). Finally, we propose a heuristic procedure---based on the notion of winding numbers of parametric curves---to efficiently compute an approximation of~these solutions with arbitrarily small~errors.


==> EC ArXiV - Upload/Sections/approx_equi.tex <==
%!TEX root = ../main.tex


In the previous section, we successfully construct a set of OUDs of the \FCB game; we now show how one can use this result to deduce an equilibrium. As a preliminary result, we give a high-level condition under which the OUDs from \cref{def:OptDis_GRCBC} constitute an equilibrium of the $\FCB$ game; it is presented as a direct corollary from \cref{theo:OUDs} as follows: 
%
 
\begin{corollary} \label{corol:FCBEqui}
    For any game $\FCBn$ and any positive solution $\kappa=(\gA, \gB)$ of System~\eqref{eq:system_f}, if there exists a mixed-strategy of Player A (resp., Player B) whose univariate marginal distributions correspond to $\Ai$ (resp., $\Bi$) for all $i \in [n]$, then these mixed strategies constitute an equilibrium of~$\FCBn$.
\end{corollary}
 
%
\cref{corol:FCBEqui} is a standard statement in analyzing equilibria of Colonel Blotto games from their OUDs. In general, it is challenging to construct such mixed strategies as required in \cref{corol:FCBEqui}---this is, as discussed in \cref{sec:Intro}, a notorious difficulty in studying the Colonel Blotto game. In the literature, several alternative concepts of solutions are proposed based on the related OUDs, they are relaxed from the equilibrium of the Colonel Blotto game in one way or another. We show that these results can also be extended to the \FCB game thanks to \cref{theo:OUDs}: in \cref{sec:GL_game}, we analyze a trivial equilibrium of the \FGL game and in \cref{sec:IU_result}, we propose an approximate equilibrium of the \FCB game based on the rescaling technique of \cite{vu2019approximate}. Nevertheless, we start in \cref{sec:Equi_FCB} by listing special cases of \FCB where the exact equilibrium can be computed.

%
%
%
%
%----------------------------------
%
 
\subsection{Exact Equilibria of the $\FCB$ Game in Particular Cases}
\label{sec:Equi_FCB}

For several parameters configurations, we can leverage existing results in special cases of the Colonel Blotto game to solve special cases of the \FCB game. For instance, \cite{roberson2006} successfully constructs an equilibrium of the game with homogeneous battlefields---the key idea is that this game has a set of OUDs that are the same for all battlefields. Therefore, we can generalize this idea to construct an equilibrium from the set of OUDs $\left\{ \Ai,  \Bi: i \in [n] \right\}$ in any $\FCBn$ game whose parameters $w_i, p_i, q_i$ are such that $ \Ai(x) = F_{A^{\kappa }_j}(x), \forall x \in [0, \infty)$, $\forall i,j \in [n]$ (and $ \Bi(x) = F_{B^{\kappa }_j}(x), \forall x \in [0, \infty)$). A simple example where this condition holds is when $w_i = w_j$, $p_i = p_j$ and $q_i = q_j $, $\forall i, j \in [n]$ in which any solution of System~\eqref{eq:system_f} induces an indices set (as defined in \cref{tab:Opt_Uni_GRCBC}) that contains the whole set $\{1, \ldots, n\}$. It is also possible to extend this approach to \FCB games where the set of battlefields can be partitioned into groups with homogeneous OUDs and such that the cardinality of each group is sufficiently large (following an idea proposed by \cite{schwartz2014} in the case of classical Colonel Blotto~games).










%
%
%------------------------------------------------
%--------------------------------------------------
 
\subsection{Equilibrium of the General Lotto Game with Favoritism}
\label{sec:GL_game}
%
In some applications of the \FCB game (and of the classical Colonel Blotto game), the budget constraints do not need to hold with probability 1; instead, they are only required to hold in expectation. In such cases, the General Lotto game with favoritism ($\FGL$) is relevant and applicable. 

%In this section, we turn our focus to the \FGL game. 
Due to the relaxation in the budget constraints, any set of OUDs of a game instance $\FCBn$ can serve as a set of equilibrium marginals of the corresponding game $\FGLn$ (having the same parameters): it is trivial to deduce mixed strategies of $\FGLn$ from univariate distributions $\Ai, \Bi, i \in [n]$ (from \cref{def:OptDis_GRCBC}). Formally, from \cref{theo:OUDs}, we have the following corollary:
%
\begin{corollary} \label{corol:payoffGL}
   For any game $\FGLn$ and any positive solution $\kappa=(\gA, \gB)$ of System~\eqref{eq:system_f}, the strategy profile where Player A (resp., Player B) draws independently her allocation to battlefield $i \in [n]$ from $\Ai$ (resp., $\Bi$) is an equilibrium.
\end{corollary}
%
% In the equilibrium of the $\FGLn$ game presented in \cref{corol:payoffGL}, the players' payoffs are 
% \begin{align}
% 	\Pi^A_{\FGL} & =  \sum \limits_{i \in I^+_1(\gA_*,\gB_*)} {\left[w_i \mathbb{I}_{\{p_i > 0\}} + \alpha w_i \mathbb{I}_{\{p_i =0\}} \right]} \! + \! \sum \limits_{i \in I^+_2(\gA_*,\gB_*)} {\left[ w_i \left(1 \!-\! \frac{q_i \gB}{\gA} \!+\! \frac{p_i}{w_i \gA} \right)  \!+\! \frac{(q_i w_i \gB \!-\! p_i )^2}{2 w_i \gA q_i \gB} \right]} \nonumber \\
% 	%
% 	& \hspace{5mm} +\!  \sum \limits_{i \in I^+_3(\gA_*,\gB_*)} \left[ \frac{w_i \gA}{2 q_i \gB} \right] \!+\! \sum \limits_{i \in I^-_2(\gA_*,\gB_*)} \left[ \frac{w_i \gA}{2 q_i \gB} \!-\! \frac{p_i ^2}{2 w_i \gA q_i \gB} \right] \!+\!  \sum \limits_{i \in I^-_3 (\gA_*,\gB_*)} \left[w_i \!-\! \frac{q_i \gB w_i }{2\gA} \right] \label{eq:payoff_A_GL},\\
% 	        \Pi^B_{\FGL} &= \sum_{i \in [n]} w_i -  	\Pi^A_{\FGL}. \label{eq:payoff_B_GL}		
% \end{align}
%
%
Naturally, in the \FGL game, when players follow the equilibrium described in \cref{corol:payoffGL}, they gain the same payoffs as in \eqref{eq:payoff_A_GL}-\eqref{eq:payoff_B_GL}. It is also trivial to check that \cref{corol:payoffGL} is consistent with previous results on the classical General Lotto game (\ie the \FGL game where $p_i=0$ and $q_i=1$ for any $i \in [n]$), \eg from \cite{myerson1993incentives,kovenock2020generalizations}.




\subsection{An Approximate Equilibrium of the \FCB Game}
\label{sec:IU_result}

In the game theory literature, approximate equilibria are often considered as alternative solution-concepts when it is impossible or inefficient to compute exact equilibria. Here, we focus on finding a good approximate equilibrium of the \FCB game that can be simply and efficiently constructed; this is relevant in applications where the budget constraints must hold precisely (\eg in security or telecommunication systems involving a fixed capacity of resources) but sub-optimality is acceptable if the error is negligible relative to the scale of the problem. We begin by recalling the definition of approximate equilibria \cite{myerson1991game,Nisan07} in the context of the \FCB game: 
%
\begin{definition}[$\eps$-equilibria]\label{def:appro_equi}
    For any $\varepsilon \ge 0$, an \emph{\mbox{$\varepsilon$-equilibrium}} of a game $\FCBn$ is any strategy profile $\left(s^{*},t^{*} \right)$ such that \mbox{$\Pi^A_{\FCBn}(s,t^*) \!\le\! \Pi^A_{\FCBn}(s^*,t^*)\!+\!\varepsilon$} and \mbox{$\Pi^B_{\FCBn}(s^*,t)\! \le\! \Pi^B_{\FCBn}(s^*,t^*)\! +\! \varepsilon$} for any strategy $s$ and $t$ of Players A and B.
\end{definition}
%
%
% Naturally, if $\varepsilon = 0$, \cref{def:appro_equi} coincides with the definition of an exact equilibrium. 


The set of OUDs constructed in \cref{sec:OptUni_GRCBC} allows us to apply directly a technique from the literature of classical Colonel Blotto game to look for an approximate equilibrium of the \FCB game: in recent work, \cite{vu2019approximate} propose an approximation scheme (called the IU strategy) for the Colonel Blotto game in which players independently draw their allocations from a set of OUDs, then rescale them to guarantee the budget constraint. The authors prove that IU strategies constitute an $\varepsilon W$-equilibrium of the CB game where $\varepsilon = \tilde{\mO}(n^{-1/2})$ and $W$ is the sum of battlefields' values. We extend this idea to the \FCB game and propose the following definition:
%
%
%
\begin{definition}[IU Strategies] \label{def:IU}
    For any game $\FCBn$ and any solution $\kappa = (\gA, \gB) \in \R^2_{>0}$ of System~\eqref{eq:system_f}, we define $\IU^{\play}_{\kappa}$ to be the mixed strategy of player $\play \in \braces*{A,B}$ such that her allocations, namely $\boldsymbol{x}^\play$, are randomly generated by the following simple procedure:\footnote{In fact, in this definition, when $\sum_{j \in [n]} a_j =0$ (resp. when $\sum_{j \in [n]} b_j =0$), we can assign any arbitrary $\boldsymbol{x}^A \in S^A$ (resp. any $\boldsymbol{x}^A \in S^B$). This choice will not affect the asymptotic results stated in this section (particularly, \cref{propo:IU}).} \emph{Player A} draws independently a real number $a_i$ from $\Ai, \forall i \in [n]$. If $\sum_{j=1}^n a_j = 0$, set $x^A_i = \frac{X^A}{n}$; otherwise, set $x^A_i = \frac{a_i}{\sum_{j=1}^n a_j} \cdot X^A$. \emph{Player B} draws independently a real number $b_i$ from $\Bi,\forall i \in [n]$. If $\sum_{j=1}^n b_j = 0$, set $x^B_i = \frac{X^B}{n}$; otherwise, set $x^B_i = \frac{b_i}{\sum_{j=1}^n b_j} \cdot X^B$.
% \begin{itemize}
%     \item 
%     %
%     \item 
% \end{itemize}
%
\end{definition}
%
Intuitively, by playing IU strategies, players draw independently from the OUDs then normalize before making the actual allocations. It is trivial to check that the realizations from $\IU^{\play}_{\kappa}$ satisfies the corresponding budget constraint in the \FCB game. Now, we consider the following~assumption:
%
\begin{assumption}\label{assum:bound}
    $\exists \wmax, \wmin: 0<\wmin \le w_i \le \wmax < +\infty$, $\forall i \in [n]$. 
\end{assumption}
%
\noindent \cref{assum:bound} is a mild technical assumption that is satisfied by most (if not all) applications of the \FCB game. Intuitively, it says that the battlefields' values of the game $\FCB$ are bounded away from 0 and infinity. With a simple adaptation of the results of \cite{vu2019approximate} (for the classical Colonel Blotto game), we obtain the following proposition (we give its proof in \ref{appen:IU}):
%
%
\begin{proposition}[IU Strategies is an $\eps$-equilibrium]
\label{propo:IU}
   In any game $\FCBn$ satisfying \cref{assum:bound}, there exists a positive number \mbox{$\varepsilon = \tilde{\mO} \left(n^{-1/2}\right)$} such that for any solution $\kappa = (\gA, \gB) \in \R^2_{>0}$ of System~\eqref{eq:system_f}, the profile $\parens*{\IU^A_{\kappa}, \IU^B_{\kappa}}$ is an \mbox{$\varepsilon W^n$-equilibrium} where $W^n:= \sum_{i=1}^n w_i$.
\end{proposition}
%
% Intuitively, if player A (resp. B) play the $\IU^A_{\kappa}$ (resp. $\IU^B_{\kappa}$), player B (resp. A) cannot unilaterally deviate from playing $\IU^B_{\kappa}$ (resp. $\IU^A_{\kappa}$) and gains more than $\eps W$.
%
Here, recall that the notation $\tilde{\mO}$ is a variant of the $\mO$-asymptotic notation where logarithmic terms are ignored. We can interpret \cref{propo:IU} as follows: consider a sequence of games $\FCBn$ in which $n$ increases (\ie games with larger and larger numbers of battlefields). Note that $W^n$ is an upper-bound of the players' payoffs in the game $\FCBn$, thus $W^n$ is relative to the scale of this game. To qualify the proposed approximate equilibrium based on the evolution of $n$, we consider the ratio between the involved approximation error $\eps W^n$ of $\parens*{\IU^A_{\kappa}, \IU^B_{\kappa}}$ and this relative-scaled quantity $W^n$; this tracks down the proportion of payoff that Player $\play$ might lose by following $\IU^{\play}_{\kappa}$ instead of the best-response against $\IU^{-\play}_{\kappa}$. As we consider $\FCBn$ games with larger and larger $n$, this ratio (which is exactly~$\varepsilon$) quickly tends to 0 with a speed in order $\tilde{\mO} (n^{-1/2})$. Therefore, in the \FCB games with large number of battlefields, the players can confidently play $\parens*{\IU^A_{\kappa}, \IU^B_{\kappa}}$ as an approximate equilibrium knowing that the involved level of error is negligible. Note also that the approximation error presented in \cref{propo:IU} also depend on other parameters of the game including $X^A, X^B$, $\wmin, \wmax$, $\max\{ \left|p_i\right|, i\in [n] \}, \min \{q_i, i \in [n]\}$ and $\alpha$ (these constants are hidden in the $\tilde{\bigoh}$ notation).





%
%
%
%
%---------------


==> EC ArXiV - Upload/Sections/conclusion.tex <==

 
 
We introduced the \emph{Colonel Blotto game with favoritism} and analyzed its equilibria and approximate equilibria. We first characterized completely the equilibrium of all-pay auctions with favoritism. Using this, we then proved that there exists a set of optimal univariate distributions of the Colonel Blotto game with favoritism and gave a construction thereof. In several special cases of the Colonel Blotto game with favoritism, these univariate distributions give an exact equilibrium; in other cases, we derived an approximate equilibrium. We then proposed an algorithm that efficiently computes an approximation of the proposed optimal univariate distributions with arbitrarily small~error. 



Our model of favoritism uses a linear-form of the winner-determination rule, defined in \cref{sec:FormCB}, similar to works on all-pay auctions with favoritism (see e.g., \cite{konrad2002investment,siegel2014asymmetric}). This is a natural formulation to capture the fundamental properties of favoritism due to its simplicity and to the natural interpretation of the parameters $p_i$ and $q_i$; and our Colonel Blotto game with favoritism---which is derived from this rule---provides a meaningful model for applications with favoritism (see \cref{sec:Intro} for several motivational examples). 
%
Nevertheless, an interesting direction for future investigations would be to consider more general winner-determination rules to model favoritism. A natural extension of our work is to consider polynomial winner-determination rules, that is, player A wins battlefield $i$ if $P^{m}_{A,i} (x^A_i) \ge P^{m}_{B,i} (x^B_i)$ and loses otherwise; where, $P^{m}_{A,i} (\cdot)$ and $P^{m}_{B,i} (\cdot)$ are some pre-determined polynomials of degree $m$ with coefficients dependent on the battlefield and the corresponding player (the first two coefficients are similar to $p_i$ and $q_i$). It would remain possible to map the corresponding Colonel Blotto game to a set of all-pay auctions; but these all-pay auctions would now have complex (polynomial) winner-determination rules. This raises two challenges: \emph{(i)} the equilibrium for such complex all-pay auctions (used to derive the optimal univariate distributions of the Colonel Blotto game) is not known and appears to be non-trivial to derive; and \emph{(ii)} proving the existence of the univariate distributions might require a fixed-point technique other than our solution in the linear-form case (cf. \cref{theo:OUDs})---or at least an adaptation of our proof technique.















==> EC ArXiV - Upload/Sections/effi_compu.tex <==
%!TEX root = ../main.tex


Our characterization of the (approximate) equilibria of the \FCB and \FGL games build upon System~\eqref{eq:system_f}. \cref{theo:OUDs} shows the existence of a solution of this system, but in practice it is also important to be able to compute such a solution. It is not clear how to do this efficiently: recall that \eqref{eq:system_f} is \emph{not} simply a system of quadratic equations in $\gA, \gB$ since as these variables change, the configuration of the indices sets (involved in the definitions of $g^A, g^B$) also changes. Given a game $\FCBn$, a naive way to solve System~\eqref{eq:system_f} would be to consider all possible partitions of \mbox{$[n]$} into $\Iplus$,  \mbox{$\Iminus$} and $[n] \backslash \bracks*{\Iplus \bigcup \Iminus}$, then solve the particular system of quadratic equations corresponding to each case. This approach, however, is inefficient as in the worst case, the number of partitions is exponential in $n$; as illustrated in the following toy example: 
% We consider \cref{ex:example_GRCB_2} as a toy example to illustrate the inefficiency of this~approach. 
%	
 
\begin{figure}[h!]
\centering
\begin{tikzpicture}
\node (img){	\includegraphics[height = 0.15\textheight]{Figures/example.png}};
\node[below=of img, node distance=0cm, yshift=1.3cm, xshift = 0.3cm] {\scriptsize $\gB$};
\node[left=of img, node distance=-0.2cm, anchor=center,yshift=-0.0cm,xshift = 0.9cm] {\scriptsize $\gA$};
\end{tikzpicture}
%
 
\caption{Conditions to partition battlefields into the indices sets of the $\FCBn$ game in \cref{ex:example_GRCB_2}.} \label{fig:example}
\end{figure}
 
\begin{example}\label{ex:example_GRCB_2}
\emph{
Consider the game $\FCBn$ with $n =2$, $X^A = X^B= 2$, $w_1 = w_2 =1$, $p_1 = -2$, $p_2 = 0$, $q_1 = 1/2$ and $q_2 = 1$.  Even in this extremely simple game, there are 6 possible configurations of $\Iplus$ and $\Iminus$. In \cref{fig:example}, we illustrate these cases by 6 regions in the first quadrant of the $\gA$-$\gB$ plane separated by the axes and the polynomials involving in the conditions that determine the indices sets. Consider these cases, each inducing a system of quadratic equations, we
%
% First, when $ 0 \le \gA, \gB \le 2$ and $ \gB \le \gA$ (i.e., when $(\gA, \gB)$ lies within Region I in \cref{fig:example}), we have $\Iplus= \{2\}$ and $\Iminus = \emptyset$. In this case, System~\eqref{eq:system_f} has a unique solution in $\mathbb{R}^2_{>0}$, which is $\gA = \gB = 4$; however, this solution does not satisfy the condition $0 \le \gA,\gB \le 2$; therefore,~\eqref{eq:system_f} has no positive solution in Region~I. Similarly, we can check for all the remaining cases. We 
%
see that there is no positive solution of~\eqref{eq:system_f} in the cases corresponding to Regions I, II, III, IV and VI of \cref{fig:example}. Only when $2 < \gA < \min \{ \gB,  \gB /2 +2 \}$ (i.e., the point $(\gA, \gB)$ lies in Region V of \cref{fig:example}), we have $\Iminus =\{1\}$ and $\Iplus=\{2\}$ and thus, System~\eqref{eq:system_f}
% 		\begin{equation*}
% 		\left\{ \begin{array}{l}
% 		(\gA)^2 /2 + (\gA - 2)^2     = 2 \gA, \\
% 		(\gA)^2 /2  + (\gA)^2 - 2^2   = 2 \gB.
% 		\end{array} \right.
% 		\end{equation*}
has a unique positive solution in $\mathbb{R}^2_{>0}$ that is $\gA = 2 + \sqrt{4/3}$ and $\gB = 2 + \sqrt{12}$ (which satisfy the conditions of Region~V).
}
%
%
%
\end{example}	
	
	
	
	
In large or even moderate instances, this naive approach is impossible, leading to the important question: can we (approximately) solve System~\eqref{eq:system_f} more efficiently? We answer this question positively: we propose in \cref{sec:approx_algo} an \emph{approximation algorithm} that computes an solution of System~\eqref{eq:system_f} with arbitrarily small error, and we analyze its running time in \cref{sec:efficiency}. Finally, in \cref{sec:approx_OUDs}, we analyze the impact of the approximation error on the OUDs from  \cref{sec:OptUni_GRCBC}. 

%An important question arises: is it possible to have more efficient methods to solve System~\eqref{eq:system_f} or to find a good approximation of its solutions? We answer this question positively. In \cref{sec:approx_algo}, we propose an \emph{approximation algorithm} that can compute an approximate solution of System~\eqref{eq:system_f} with arbitrarily small error. In \cref{sec:efficiency}, we analyze the efficiency and scalability of the proposed approximation~algorithm. Finally, in \cref{sec:approx_OUDs}, we analyze the relation between outputs of our approximation algorithm and the set of OUDs proposed in \cref{sec:OptUni_GRCBC}. 




%
%
%
%----------------------
\subsection{An Approximation Algorithm Solving System~\eqref{eq:system_f}}
\label{sec:approx_algo}
 %
Throughout this section, we focus on the following approximation concept: in any game $\FCBn$ (and $\FGLn$), for any $\delta>0$,  a point $(\tgA, \tgB) \in \mathbb{R}^2_{>0}$ is called a \emph{${\delta}$-approximate solution} of System~\eqref{eq:system_f} if there exists a solution $(\gA, \gB) \in \R^2_{>0}$ of System~\eqref{eq:system_f} satisfying the following conditions:
	%
\begin{align}
    %
    	& \left| \tgA - \gA \right| \le {\delta} \textrm{ and }  \left|\tgB - \gB \right| \le {\delta}, \label{eq:delta_close} \\
    	%
        \textrm{ and }&  g^A(\tgA, \tgB)\le 0 \textrm{ and } g^B(\tgA, \tgB)\le0. \label{eq:system_approx_f}
\end{align}
%
Intuitively, any $\tk = (\tgA, \tgB)$ satisfying~\eqref{eq:delta_close} is ${\delta}$-close to a solution of System~\eqref{eq:system_f} (in the metric induced by the $\| \cdot\|_{\infty}$ norm) and, by \eqref{eq:system_approx_f}, the distributions $\braces*{ \tAi, \tBi , i \in [n]}$ from \cref{def:OptDis_GRCBC} corresponding to $\tk$ satisfies Condition~\ref{condi:OUD2} of \cref{def:OUD} (i.e., budget constraints).\footnote{Note also that since $G$ is continuous (it is also Lipschitz-continuous \wrt $\| \cdot \|_{\infty}$ norm), the distance between $G(\tgA, \tgB)$ and $(0,0)$ also tends to 0 when $\delta \rightarrow 0$; to quantify this, one might look for the Lipschitz constants of $g^A, g^B$; but since this analysis is not relevant to results presented in this section, we omit the details.} In principle, we would like to find ${\delta}$-approximate solutions such that $\delta$ is as small as possible; naturally, this will come with a trade-off on the running time (we discuss this further in \cref{sec:efficiency}). 



We propose an approximation algorithm, having a stopping-criterion parameter $\delta$, that quickly finds a $\delta$-approximate solution of~\eqref{eq:system_f} in any game $\FCBn$. A pseudo-code of this algorithm is given in \ref{appen:heuristic} along with many details; we discuss here only its main intuition. Recall that the function $G:\R^2 \rightarrow \R^2$ defined in~\eqref{eq:G_func} is a continuous mapping and that solving System~\eqref{eq:system_f} is equivalent to finding a zero of $G$. To do this, our approximation algorithm consists of a dichotomy procedure (i.e., a bisection method) such that at each loop-iteration, it considers a smaller subset of $\mathbb{R}^2$. It starts with an arbitrary rectangle $D \subset \mathbb{R}^2_{>0}$ (including its boundary and interior), then checks to see whether its image via $G$ contains the point $(0,0)$---this can be done by computing the winding number of the $G$-image of the boundary of $D$ (which is a closed parametric curve) around $(0,0)$: due to \cref{lem:wind}, if this winding number is non-zero, $G(D)$ contains $(0,0)$. If $G(D)$ does not contains $(0,0)$, we enlarge the rectangle $D$ (\eg by doubling its length and width) while maintaining that $D \subset \R^2_{>0}$. We repeat this enlargement step until we find a rectangle whose $G$-image contains $(0,0)$. Due to \cref{theo:OUDs} and \cref{lem:wind}, such a rectangle $D$ exists with a zero of $G$ inside. We then proceed by dividing the rectangle $D$ into smaller rectangles and checking which among them has a $G$-image containing $(0,0)$, then repeating this procedure on that smaller rectangle. The algorithm terminates as soon as it finds a rectangle, say $D^*$, such that $G(D^*)$ has a non-zero winding number around $(0,0)$ and $D^*$ has a diameter smaller than $\delta$ (thus any point in $D^*$ satisfies \eqref{eq:delta_close}); as a sub-routine of the computation of the involved winding number, our algorithm also determines a point $(\tgA, \tgB)$ in $D^*$ satisfying \eqref{eq:system_approx_f}. The output $(\tgA, \tgB)$ is a $\delta$-approximate solution of System~\eqref{eq:system_f}.





%
%
%---------------------------------
%---------------------------------
\subsection{Computational Time of the Approximation Algorithm}
\label{sec:efficiency}
In the approximation algorithm described above, the most complicated step is the computation of the winding number of the involved rectangles. To do this efficiently, we draw tools from the literature: for any parametric curve $\curve:[a,b] \rightarrow \R^2$ where $\min_{t \in [a,b]} \| \curve(t)\|_{\infty} = \delta$, the insertion procedure with control of singularity (IPS) algorithm proposed by \cite{zapata2012geometric} takes $\bigoh \parens*{(b-a) \delta^{-1}}$ time to output a special polygonal approximation of $\curve$---having a number $\bigoh \parens*{(b-a) \delta^{-1}}$ of vertices---such that the winding number of this polygonal approximation is precisely the winding number of $\curve$. To compute this winding number, we calculate the value of $\curve$ at all vertices of this polygon. Inserting IPS into our approximation algorithm running with the parameter $\delta$, in any game $\FCBn$, for any rectangle~$D$ in consideration, we can represent $G(\partial D)$ by a parametric curve $\curve:[a,b] \rightarrow \R^2$ and compute the winding number of $G(\partial D)$ in $\bigoh \parens*{n(b-a) \delta^{-1}}$ time (it takes $\bigoh(n)$ time to compute the $G$-value of a vertex of the polygonal approximation). Note that this computational time also depends on other parameters of the game $\FCBn$ (they are hidden in $\bigoh$-notation above); we discuss this point in details in \ref{appen:heuristic}. Based on this procedure, we have the following~proposition:
%
% \begin{proposition}\label{propo:heuristic}
%     Let $(\gA, \gB) \in \mathbb{R}^2_{>0}$ be a solution of System~\eqref{eq:system_f} such that 
% \end{proposition}
%

\begin{proposition}\label{propo:heuristic}
    For any game $\FCBn$ and $\delta <1$, the approximation algorithm described above finds a $\delta$-approximate solution of System~\eqref{eq:system_f} in $\tilde{\bigoh}(n \delta^{-1})$ time.
\end{proposition}
%
%
\cref{propo:heuristic} confirms the efficiency of our approximation algorithm, as the running time of our algorithm is only $\bigoh(n)$. The order $\tilde{\bigoh}(\delta^{-1})$ gives the trade-off between the running-time and the precision-level of solutions $\delta$. In fact, the running time of our algorithm also depends on the choice of the initial rectangle. More precisely, for a solution $(\gA, \gB)$ of System~\eqref{eq:system_f} such that \mbox{$\|(\gA, \gB)\|_{\infty} \!<\!R$}, our approximation algorithm, initialized with a rectangle whose center $(\gA_0,\gB_0)$ satisfying $\|(\gA_0,\gB_0) \|_{\infty} =  L_0$ and $\delta <1$, terminates after $\bigoh \parens*{\log \parens*{\frac{R}{\delta}} + \log \parens*{ \max \braces*{\frac{R}{L_0}, \frac{L_0}{R}}}}$ iterations and each iteration runs in $\bigoh \parens*{ {R n}{\delta}^{-1} }$ time. Intuitively, if the initialized rectangle is too small and/or the actual solution is too far away from this rectangle, the algorithm requires a longer time. We conduct several experiments to illustrate the computational time of our approximation algorithm. Due to space constraints, we place these results in~\ref{appen:heuristic}; globally, our proposed algorithm is very fast in comparison with the naive approach described~above.

% \begin{example}
%     \emph{Recall the game instance $\FCBn$ (with $n=2$) considered in \cref{ex:example_GRCB_2} where System~\eqref{eq:system_f} has one positive (exact) solution $(\gA,\gB) := (2 + \sqrt{4/3}, 2+\sqrt{12}) \approx (3.1547005,5.4641016) $. With the parameter \mbox{$\delta=10^{-6}$}, our approximation algorithm outputs the solution $(\tgA, \tgB) =( 3.1547010, 5.4641018) $. The computation time is $\sim 2.78$~seconds when initializing with the rectangle whose vertices are $(\delta,\delta)$, $(\delta, 10X^A)$, $(10X^A, 10X^A)$ and~$(10X^A,\delta)$.}
% \end{example}
%%
%
% Besides this toy example, we also conduct several experiments to illustrate the computational time of our approximation algorithm. Due to space constraints, we place these results in~\ref{appen:heuristic}; globally, our proposed algorithm is very fast in comparison with the naive approach described~above. 
% For example, it takes merely $10$ seconds to find a \emph{$\delta$-approximate solution} when we choose $\delta =  10^{-6}$ of System~\eqref{eq:system_f} corresponding to an instance of a $\FCBn$ game with $n = 100$.
%

	
 
%
%
%-----------------------------------
%----------------------------------
\subsection{Approximations of Optimal Univariate Distributions of the \FCB Game}
\label{sec:approx_OUDs}
%	
%	
To conclude this section, we show that from a $\delta$-approximate solutions of System~\eqref{eq:system_f}, one gets an approximate equilibrium  for the \FCB and \FGL games. This is based on the following proposition:
%The proposed approximation algorithm not only efficiently find $\delta$-approximate solutions of System~\eqref{eq:system_f}, but it is also relevant and useful thanks to the following important lemma:
  
\begin{proposition}\label{lem:approx_sol}
    In any game $\FCBn$ (and $\FGLn$), let $\kappa = (\gA,\gB)$ and $\tk = (\tgA, \tgB)$ be a positive solution and a $\delta$-approximate solution of System~\eqref{eq:system_f} respectively (such that $\kappa, \tk$ satisfy \eqref{eq:delta_close}-\eqref{eq:system_approx_f}). Then, the sets of distributions $\braces{\Ai,\Bi, i \in [n]}$ and $\braces{\tAi,\tBi, i \in [n]}$ from \cref{def:OptDis_GRCBC} corresponding to $\kappa$ and $\tk$~satisfy $\big| \Ai(x)\! -\! \tAi(x) \big| \le \bigoh \parens{\delta}$ and $\big| \Bi(x) - \tBi(x) \big| \le \bigoh\parens{\delta}$, for any $i \in [n]$ and~$x\in [0,\infty)$. 
\end{proposition}
%
%
A proof of \cref{lem:approx_sol} is given in \ref{appen:approx_OUD}. Intuitively, it shows that when $\tk = (\tgA, \tgB)$ is a $\delta$-approximate solution of \eqref{eq:system_f}, the distributions ${\tAi,\tBi}$ are approximations of the distributions ${\Ai,\Bi}$ with the approximation error in order $\bigoh(\delta)$ (note that it is also polynomial in terms of $1/\min\{\gA, \tgA, \gB, \tgB\}$, $\max\{\gA, \tgA, \gB, \tgB\}$, $1/\min_{i \in [n]}{q_i}$ and $\max_{i \in [n]}{|p_i|}$). From \cref{lem:approx_sol}, we can also deduce that the players' payoffs when they use strategies with marginals following ${\tAi,\tBi, i \in [n]}$ are $\bracks*{\bigoh ( \delta) W^n}$-close to the payoffs when players use strategies with marginal ${\Ai,\Bi, i \in [n]}$ (see the formulations given in \eqref{eq:payoff_A_GL}-\eqref{eq:payoff_B_GL}). As a consequence, by following the scheme leading to results in \cref{sec:Corollary_results}, for any games $\FCBn$ and $\FGLn$ (having the same parameters), for any $\delta$-approximate solution $\tk = (\tgA, \tgB)$ of System~\eqref{eq:system_f}, we have:
%
\begin{itemize}
    \item[$(i)$] In $\FGLn$, the strategies profile when Player A (resp. Player B) draws independently her allocation to battlefield $i$  from ${\tAi}$ (resp. $\tBi$) constitutes a $\bracks*{\bigoh(\delta) W^n}$-equilibrium.\footnote{These are indeed mixed strategies of $\FGLn$ since $\sum_{i \in [n]} \Ex_{x \sim \tAi} \left[ x  \right] < X^A$ and $\sum_{i \in [n]} \Ex_{x \sim \tBi} \left[ x  \right] < X^B$ due to~\eqref{eq:system_approx_f}.}
    %
    \item[$(ii)$] In $\FCBn$, the strategies $(\IU^{A}_{\tk}, \IU^{B}_{\tk} )$ is a $\bracks*{\bigoh(\delta + \varepsilon ) W^n}$-equilibrium where $\varepsilon = \tilde{\bigoh}(n^{-1/2})$. In this case, we
    cannot obtain an approximate equilibrium with a level of error better than $\varepsilon$; to achieve this, we only need to run the approximation algorithm with $\delta = {\varepsilon}$.
\end{itemize}
	%	
	% 	\begin{figure}[h!]
	% 		\centering
	% 		\begin{tikzpicture}
	% 		\node (img){\includegraphics[height = 0.18\textheight]{Figures/p_runs.png}};
	% 		\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = 0.3cm] {$p$};
	% 		\node[left=of img, node distance=0cm, rotate=90, anchor=center,yshift=-0.7cm] {Expected payoff of Player A};
	% 		\end{tikzpicture}
	% 		%
	% 		\caption[]{Expected payoff of Player A when players follow the equilibrium in instances of \FGL games where $n=4$, $X^A = X^B = 10$, $\alpha = 1/2$; each battlefield $i$ has $w_i = 1$ and $p_i = p$.} \label{fig:p_runs}
	% 	\end{figure}
	
	
	
	% 	\begin{figure}[h!]
	% 		\centering
	% 		\begin{tikzpicture}
	% 		\node (img){\includegraphics[height = 0.4\textwidth]{Figures/q_runs.png}};
	% 		\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = 0.1cm] {$q$};
	% 		\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift = 0.2cm,yshift = -0.7cm] {Expected payoff of Player A};
	% 		\end{tikzpicture}
	% 		%
	% 		\caption[]{Expected payoff of Player A when players follow the equilibrium in instances of \FGL games where $n=4$, $X^A = X^B = 10$, $\alpha = 1/2$; each battlefield $i$ has $w_i = 1$ and $q_i=q$.} \label{fig:q_runs}
	% 	\end{figure}

==> EC ArXiV - Upload/Sections/equi_APA.tex <==
%!TEX root = ../main.tex



In this section, we characterize the equilibrium of the $\FAPA$ game. The closed-form expression of the equilibrium depends on the relation between the parameters $u^A, u^B,p$ and $q$. We present two groups of results corresponding to two cases: $p \ge 0$ (\cref{sec:APAPos}) and $p<0$ (\cref{sec:APANeg}). 



%
%
%-----------------------------------------------
\subsection{Equilibria of $\FAPA$ with $p \ge 0$.}
\label{sec:APAPos}
%
We first focus on the case where $p \ge 0$; in other words, Player A has an additive advantage. In equilibrium, players choose their bids according to uniform-type distributions which depend on the relation between $u^A, u^B, p$ and $q$. Particularly, we obtain the following theorem:
%	
%	
\begin{theorem}
\label{theo:positive}
In the $\FAPA$ game where $p \ge 0$, we have the following results:
	
\begin{itemize}
    \item[$(i)$] If $q u^B - p \le 0$, there exists a unique pure equilibrium where players' bids are $x^A = x^B = 0$ and their equilibrium payoffs are $\mathrm{\Pi}^A_{\FAPA} = u^A$ and $\mathrm{\Pi}^B_{\FAPA} = 0$ respectively.
	%
	\item[($ii$)] If $0 < q u^B - p \le u^A$, there exists no pure equilibrium; there is a unique mixed equilibrium where Player A (resp. Player B) draws her bid from the distribution $\Aiip$ (resp. $\Biip$) defined as follows.
	\begin{align}
	& \Aiip(x) =   \left\{ \begin{array}{l}
	\frac{p}{q u^B} + \frac{x}{q u^B}, \forall x \in \left[ 0, q u^B \!-\! p \right], \\
	1                  \qquad \qquad, \forall x > q u^B \!-\!p, 
	\end{array} \right.
	%
	\textrm{and} 
	%
	& \Biip(x) =   \left\{ \begin{array}{l}
	1 - \frac{q u^B}{u^A} + \frac{p}{u^A}, \forall x \in \left[ 0, \frac{p}{q} \right) \\
	1 - \frac{q u^B}{u^A} + \frac{q \cdot x}{u^A}, \forall x \in \left[\frac{p}{q}, u^B \right], \\
	1 \qquad \qquad \qquad, \forall x > u^B.
	\end{array} \right. \label{eq:A+Def}
	\end{align}
	In this mixed equilibrium, players' payoffs are $\mathrm{\Pi}^A_{\FAPA} = u^A - q u^B + p$ and $\mathrm{\Pi}^A_{\FAPA} =0$.
	%
	%
	\item[$(iii)$]  If $q u^B - p > u^A$, there exists no pure equilibrium; there is a unique mixed equilibrium where Player A (resp. Player B) draws her bid from the distribution $\Aiiip$ (resp. $\Biiip$) defined as follows.
	\begin{align}
	& \Aiiip(x) =   \left\{ \begin{array}{l}
	1- \frac{u^A}{q u^B} + \frac{x}{q u^B}, \forall x \in \left[ 0, u^A \right], \\
	1          \qquad  \qquad \qquad, \forall x > u^A, 
	\end{array} \right.
	%
	\textrm{ and } 
	%
	& \Biiip(x) =   \left\{ \begin{array}{l}
	0 \qquad \qquad, \forall x \in \left[ 0, \frac{p}{q} \right) \\
	- \frac{p}{u^A} + \frac{q \cdot x}{u^A}, \forall x \in \left[\frac{p}{q}, \frac{u^A + p}{q} \right], \\
	1 \qquad \qquad, \forall x > \frac{u^A + p}{q}.
	\end{array} \right. \label{eq:bFA+Def}
	\end{align}
	In this mixed equilibrium, players' payoffs are $\mathrm{\Pi}^A_{\FAPA}= 0$ and $\mathrm{\Pi}^B_{\FAPA} = u^B - (u^A+p)/q$.
			
	\end{itemize}
\end{theorem}
	
A formal proof of \cref{theo:positive} can be found in \ref{appen:proofAPAPos}; here we discuss an intuitive interpretation of the result. First, note that no player has an incentive to bid more than the value at which she assesses the item, otherwise she is guaranteed a negative payoff. Then, the condition in Result~$(i)$ of \cref{theo:positive} indicates that Player A has too large advantages such that she always wins regardless of her own bid and Player B's bid, hence it is optimal for both players to bid zero (see the proof for the case $q u^B - p =0$). The condition in Result~$(ii)$ of \cref{theo:positive} gives Player A a favorable position: she can guarantee to win with a non-negative payoff by bidding $u^A$ knowing that Player B will not bid more than $u^B$; reversely, the condition in Result~$(iii)$ implies that Player B has a favorable position: by bidding $u^B$, she guarantees to win with a non-negative payoff since Player A will not bid more than $u^A$. Importantly, in Result~$(ii)$ of this theorem, as long as the condition $0 < q u^B - p \le u^A$ is satisfied, when $p$ increases (and/or $q$ decreases), the equilibrium payoff of Player A increases. This is in coherence with the intuition that when Player A has larger advantages, she can gain more. However, if $p$ is too large (and/or $q$ is too small) such that the condition in Result~$(i)$ of \cref{theo:positive} is satisfied, Player B gives up totally and Player A gains a fixed payoff ($u^A$) even if $p$ keeps increasing (and/or $q$ keeps decreasing). A similar intuition can be deduced for Player B and~Result~$(iii)$.
%	First, we observe that in all equilibria, Player A does not bid more than $\min \{u^A, q u^B - p \}$ and Player B does not bid more than $\min\{u^B, (u^A + p)/q\}$. This can be explained by the observation that \emph{no player has an incentive to bid more than the value} she assesses on the item: if Player A (resp. Player B) bids strictly more than $u^A$ (resp. $u^B$), she surely receives a negative payoff (even if she wins the item); on the other hand, by bidding $0$, she can always guarantee to have a non-negative payoff.\footnote{That is \mbox{$\Pi^A_{\FAPA}\left( x^A, x^B \right) < 0, \forall x^A > u^A, \forall x^B$} while $\Pi^A_{\FAPA}\left(0, x^B \right) \ge 0$ and similarly, \mbox{$\Pi^B_{\FAPA}\left( x^A, x^B \right) < 0, \forall x^A, \forall x^B > u^B$} while \mbox{$\Pi^B_{\FAPA}\left(x^A,0 \right) \ge 0$}} Knowing this, Player A (resp. Player B) does not need to bid more than $q u^B -p$ (resp. $(u^A + p)/q$) in order to win the item. 


%\footnote{It is trivial to verify that the functions $\Aiip, \Biip,\Aiiip$ and $\Biiip$ satisfy the conditions of being distributions (under the corresponding conditions of the game's parameters in each case).}
\begin{figure*}[htb!]
\centering
\subfloat[$\FAPA$ instance with $u^A = 4$, $u^B = 2$, \mbox{$p = 1.5$}, $q =1.5$ (i.e., \mbox{$0 \le q u^B-p < u^A$}). ]{
	\begin{tikzpicture}
	\node (img){\includegraphics[height=0.20\textwidth]{Figures/I+2.png}};
	\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = 0.5cm] {\scriptsize$x$};
	%   \node[left=of img, node distance=0cm, rotate=90, anchor=center,yshift=-0.7cm] {y-axis};
	\end{tikzpicture}
}   
\qquad \qquad
%
\subfloat[$\FAPA$ instance with $u^A = 2$, \mbox{$u^B = 4$}, \mbox{$p = 1$}, $q =1$ (i.e., \mbox{$ q u^B-p > u^A$}). ]{
	\begin{tikzpicture}
	\node (img){\includegraphics[height=0.205\textwidth]{Figures/I+3.png}};
	\node[below=of img, node distance=0cm, yshift=1.1cm,xshift = 0.5cm] {\scriptsize$x$};
	%   \node[left=of img, node distance=0cm, rotate=90, anchor=center,yshift=-0.7cm] {y-axis};
	\end{tikzpicture}
}%
\caption{The mixed equilibrium of the $\FAPA$ with $p\ge 0$.}
\label{fig:APA_pos}
\end{figure*}

We now turn our focus to the distributions $\Aiip, \Biip,\Aiiip$ and $\Biiip$ in Results~$(ii)$ and~$(iii)$ of \cref{theo:positive}. First, note that the superscript ${}^+$ in the notations of these distributions simply refers to the condition $p \ge 0$ being considered (to distinguish it with the case where $p < 0$ presented below) while the subscript index ($2$ or $3$) indicates that these distributions correspond to Results~$(ii)$ or~$(iii)$. These distributions all relate to uniform distributions: $\Aiip$ is the distribution placing a non-negative probability mass at zero, and then uniformly distributing the remaining mass on the range $\left(0, q u^B-p \right]$ while $\Biip$ places a non-negative mass at zero, then uniformly distributes the remaining mass on $\left[p/q,u^B \right]$; similarly, $\Aiiip$ places a mass at zero and uniformly distributes the remaining mass on $\left( 0, u^A \right]$ while $\Biiip$ is the uniform distribution on $\left[p/q, (u^A+p)/q \right]$; see  an illustration in \cref{fig:APA_pos}. Note finally that \cref{theo:positive} is consistent with results in the restricted cases of \FAPA presented in \cite{konrad2002investment} (where $u^A = u^B$, $p \ge 0$, $0 < p <1$ and $\alpha =1/2$) and with results for the classical APA from \cite{baye1996all,hillman1989} (i.e., when $p =0$, $q = 1$, $\alpha = 1/2$); see \ref{appen:preli} where we reproduce these results to ease comparison. 
%
%
%

	



%\footnote{For the sake of reference, we rewrite the relevant results extracted from \cite{baye1996all} and \cite{konrad2002investment} in \ref{appen:preli}.}
 
 



	
	
	
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The $\FAPA$ game with $p < 0$}
\label{sec:APANeg}
%
We now consider the $\FAPA$ game in the case $p < 0$. We first define $p^{\prime} = -p/q$ and $q^{\prime} = 1/q$. Since $p<0$, we have $p^{\prime} >0$. Moreover, \mbox{$\be \left(x^A, q x^B - p \right) = \be \left( (x^A +p)/q, x^B\right) = \be \left(  q^{\prime} x^A - p^{\prime}, x^B \right)$} for any $x^A, x^B$. Therefore, the $\FAPA$ game with $p < 0$ (and $q>0$) is equivalent to an \FAPA with $p^{\prime} >0 $ (and $q^{\prime} >0$) in which the roles of players are exchanged. Applying \cref{theo:positive} with $p^{\prime}>0$ (and $q^{\prime} >0$), we can easily deduce the equilibrium of the \FAPA with $p<0$. Due to the limited space, we only present this result in \ref{sec:appen:APAneg}.
	
%\footnote{The tie-breaking rule does not change, i.e., in cases where $ q^{\prime} x^A - p^{\prime} =  x^B$, Player A gains $\alpha u^A $ and Player B gains $(1- \alpha) u^B $.}
	
	
	
	
	
	
	
	
	

==> EC ArXiV - Upload/Sections/equi_FCB.tex <==
%!TEX root = ../main.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%
The notion of optimal univariate distributions plays a key role in the equilibrium characterization of the Colonel Blotto game and its variants. In this section, we prove the existence of, and construct a set of optimal univariate distributions of the $\FCB$ game. This is the core result of our work.

%
%
%
%-------------------------

	
% %
% \begin{align*}
% I^+_1(\gA, \gB) &:= \left\{i \in [n]:p_i \ge 0, q_i w_i \gB \!-\! p_i \le 0  \right\}, \\
% %
% I^+_2(\gA, \gB) &:= \left\{i \in [n]: p_i \ge 0, 0< q_i w_i \gB \!-\! p_i \le w_i \gA  \right\}, \\
% %
% I^+_3(\gA, \gB) &:= \left\{i \in [n]: p_i \ge 0, q_i w_i \gB \!-\! p_i > w_i \gA \right\}, \\
% %
% I^-_1(\gA, \gB) &:= \left\{i \in [n]: p_i <0, {w_i \gA}  \le - p_i \right\}, \\
% %
% I^-_2(\gA, \gB) &:= \left\{i \in [n]: p_i <0, -p_i< {w_i \gA} \le q_i w_i \gB \!-\! p_i \right\}, \\
% %
% I^-_3(\gA, \gB) &:= \left\{i \in [n]: p_i <0, {w_i \gA } > q_i w_i \gB \!-\! p_i \right\}.
% %
% \end{align*}
% %
% It is easy to see that for any $(\gA, \gB) \in \mathbb{R}^{2}_{\ge 0}$, these sets are disjoint and their union is $\{1,2,\ldots,n\}$ (corresponding to $n$ battlefields in $\FCBn$). Hereinafter, we refer to these six sets as \emph{indices sets}. 
% In the notation of these sets, the superscript ${}^+$ (resp. ${}^-$) implies that they include battlefield $i$ with the corresponding parameter $p_i \ge 0$ (resp. $p_i <0$). 
% On the other hand the subscript $j \in \{1,2, 3\}$ in the notations $I^+_j$ (resp. notations $I^-_j$) indicates that the conditions in $I^+_j$ (resp. $I^-_j$) corresponds to the conditions in the Results~$(i)$, $(ii)$ or $(iii)$ of \cref{theo:positive} (resp. \cref{theo:negative} on equilibria of \Fall-pay auctions with $p <0$---see Appendix~\ref{sec:appen:APAneg}) where we replace $p = p_i, q = q_i$, $u^A = w_i \cdot \gA$ and $u^B = w_i \cdot \gB$.


%it is not necessary to state the particular parameters $\gA, \gB$, we lighten the notation by writing $I^+_j$ and $I^-_j$ instead of $I^+_j(\gA,\gB)$ and~$I^-_j(\gA,\gB)$ for $j \in \{1,2,3\}$. Now, based on these indices sets, we give the following definition.
%
As discussed in \cref{sec:Intro}, a classical approach in the Blotto games literature is to reduce the problem of constructing optimal univariate distributions (OUDs) to the problem of finding the equilibria of a set of relevant all-pay auction instances---each corresponding to players' allocations in one battlefield. The main question then becomes: \emph{which set of all-pay auction instances should we consider in order to find OUDs of the $\FCB$ game?} Naturally, from their formulations in \cref{sec:FormCB} and \cref{sec:FormAPA}, a candidate is the set of $\FAPA$ games in which the additive and multiplicative advantages of the bidders correspond to the parameters representing the pre-allocations and asymmetric effectiveness of players in each battlefield of the $\FCB$ game. The (uniquely defined) equilibrium distributions of these $\FAPA$ games satisfy Condition~\ref{condi:OUD3} in \cref{def:OUD} (\ie they are the marginal best-response against one another in the corresponding battlefield of the $\FCB$ game). Now, we only need to define the items' values in these $\FAPA$ games in such a way that their corresponding equilibrium distributions also hold Condition~\ref{condi:OUD2} in \cref{def:OUD} (\ie they satisfy the budget constraints in expectation). To do this, we first parameterize the items' values assessed by the bidders in the involved $\FAPA$ games, then we match these parameters with equations defining Condition~\ref{condi:OUD2}. Summarizing the above discussion, we define a particular set of distributions (on $\Rpos$) as~follows:
%
%	
\begin{definition}	\label{def:OptDis_GRCBC}
		Given a game $\FCBn$ and a pair of positive real numbers $\kappa = (\gA, \gB)\! \in\! \mathbb{R}^{2}_{> 0}$, for each $i\! \in\! [n]$, we define $\Ai$ and $\Bi$ to be the pair of distributions that forms the equilibrium of the $\FAPA$ game with $p:= p_i$, $q:= q_i$, $u^A:= w_i \cdot \gA$ and $u^B:= w_i \cdot \gB$. The explicit formulas of $\Ai$ and $\Bi$ are given in \cref{tab:Opt_Uni_GRCBC} for each configuration of $w_i, p_i, q_i, \gA$ and $\gB$.	
	\end{definition}
	%
	\begingroup
	\renewcommand{\arraystretch}{1.2} % Default value: 1
	\begin{table}[tb!]
	\footnotesize
		\centering
		\caption[]{$\Ai$ and $\Bi$ corresponding to $\kappa  =  (\gA, \gB)$ and a $\FCBn$ game. The notation $I^+_j(\gA,\gB)$ and $I^-_j(\gA,\gB)$ for $j=1,2,3$ denote the set of indices of battlefields satisfying the corresponding conditions; for example, $I^+_1(\gA, \gB)=\{i  \in  [n]:p_i \ge 0, q_i w_i \gB - p_i \le 0\}$ and $\forall i \in I^+_1 (\gA, \gB)$, $\Ai(x)  = 1$, $\Bi(x)  = 1, \forall x~\ge~0$.} \label{tab:Opt_Uni_GRCBC}
		\begin{tabular}{ |l|l|l| } 
			\hline
			\rowcolor{Gray}
			Indices Sets & Conditions & Definition  \\
			\hline
			%%%%%%%%%%%%%%%%%%%%55 I+1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
			$I^+_1(\gA, \gB)$ &  {$i  \in  [n]:p_i \ge 0$, $q_i w_i \gB - p_i \le 0$}      & $\Ai(x)  = 1, \forall x \ge 0$ and $\Bi(x)  = 1, \forall x \ge 0$.   \\ 
			\hline
			%%%%%%%%%%%%%%%%%%  I+2  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			%
			$I^+_2(\gA, \gB)$ & \multirow{2}{3cm}{$i  \in  [n]: p_i \ge 0$, \mbox{$0 < q_i w_i \gB  -  p_i  \le  w_i \gA$}}  
			%
			& $\Ai(x)  =  \left\{ \begin{array}{l}
			\frac{p_i}{q_i w_i \gB} +  \frac{x}{q_i w_i \gB}, \forall x  \in  \left[ 0, q_i w_i \gB  -  p_i \right], \\
			1              \qquad  \quad  \qquad \qquad, \forall x > q_i w_i \gB -p_i, 
			\end{array} \right.$     \\      
			%
			%
			& & $\Bi(x)  = \left\{ \begin{array}{l}
			1 - \frac{q_i \gB}{\gA} +  \frac{p_i}{w_i \gA}, \forall x  \in  \left[ 0, \frac{p_i}{q_i} \right), \\
			1 - \frac{q_i \gB}{\gA} +  \frac{q_i \cdot x}{w_i \gA}, \forall x  \in  \left[\frac{p_i}{q_i}, w_i \gB \right], \\
			1 \qquad \quad \qquad \qquad, \forall x > w_i \gB.
			\end{array} \right.$   \\ 
			%%%%%%%%%%%%%%%%%%%     I+3    %%%%%%%%%%%%%%%%%%%%5
			\hline
			\ %
			$I^+_3(\gA, \gB)$ & \multirow{2}{3cm}{$i  \in  [n]: p_i \ge 0$, \mbox{$q_i w_i \gB - p_i > w_i \gA$}}  
			%
			& $\Ai(x)  =    \left\{ \begin{array}{l}
			1- \frac{\gA}{q_i \gB} +  \frac{x}{q_i w_i \gB}, \forall x  \in  \left[ 0, w_i \gA \right], \\
			1         \qquad \qquad  \qquad \qquad, \forall x > w_i \gA, \end{array} \right.$\\
			%
			& & $\Bi(x)  =    \left\{ \begin{array}{l}
			0 \qquad \qquad \qquad, \forall x  \in  \left[ 0, \frac{p_i}{q_i} \right), \\
			- \frac{p_i}{w_i \gA} +  \frac{q_i \cdot x}{w_i \gA}, \forall x  \in  \left[\frac{p_i}{q_i}, \frac{w_i \gA +  p_i}{q_i} \right], \\
			1 \qquad \qquad \qquad, \forall x > \frac{w_i \gA +  p_i}{q_i}.
			\end{array} \right.  $ \\ 
			%%%%%%%%%%%%%%%%%%%%%   I-1  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\hline
			$I^-_1(\gA, \gB)$  & {$i  \in  [n]: p_i <0$, ${w_i \gA}  \le - p_i$}      & $\Ai(x)  = 1, \forall x \ge 0$ and $\Bi(x)  = 1, \forall x \ge 0$. \\ 
			\hline
			%%%%%%%%%%%%%%%%%%  I-2  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			%
			$I^-_2(\gA, \gB)$ & \multirow{2}{3cm}{$i  \in  [n]: p_i <0$, \mbox{$-p_i< {w_i \gA} \le q_i w_i \gB  -  p_i$}}  
			%
			& $\Ai(x)  = \left\{ \begin{array}{l}
			1-\frac{\gA}{q_i \gB} - \frac{p_i}{q_i w_i \gB}, \forall x  \in  \left[ 0, - p_i \right), \\
			1-\frac{\gA}{q_i \gB} +  \frac{x}{q_i w_i \gB}, \forall x  \in  \left[ -p_i, w_i \gA \right],\\
			1             \qquad  \quad   \qquad \qquad, \forall x > w_i \gA, 
			\end{array} \right.$         \\ 
			%
			&  & $\Bi(x) : \left\{ \begin{array}{l}
			- \frac{p_i}{w_i \gA} +  \frac{q_i \cdot x}{w_i \gA}, \forall x  \in  \left[ 0, \frac{w_i \gA +  p_i}{q_i} \right], \\
			1 \qquad \qquad \qquad, \forall x > \frac{w_i \gA +  p_i}{q_i}.
			\end{array} \right.$   \\ 
			%%%%%%%%%%%%%%%%%%%     I-3    %%%%%%%%%%%%%%%%%%%%5
			\hline
			\ %
			$I^-_3(\gA, \gB)$ & \multirow{2}{3cm}{$i  \in  [n]: p_i <0$, \mbox{${w_i \gA } > q_i w_i \gB  -  p_i$}}  
			%
			& $\Ai(x)  =   \left\{ \begin{array}{l}
			0 \qquad \quad \qquad \qquad, \forall x  \in  \left[ 0, -p_i \right), \\
			\frac{p_i}{q_i w_i \gB} +  \frac{x}{q_i w_i \gB}, \forall x  \in  [  - p_i, q_i w_i \gB  -  p_i],\\
			1 \qquad \quad \qquad , \forall x > q_i w_i \gB -p_i,
			\end{array} \right.$ \\ 
			%
			& & $\Bi(x)  =   \left\{ \begin{array}{l}
			1- \frac{q_i \gB}{\gA} +  \frac{q_i \cdot x}{w_i \gA}, \forall x  \in  \left[0, w_i \gB \right], \\
			1 \qquad \quad \qquad \qquad, \forall x > w_i \gB.
			\end{array} \right. $\\
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\hline
		\end{tabular}
	\end{table}
\endgroup
%
%
%
We consider the following system of equations (with variables~$\gA, \gB$):
\begin{align}
	\left\{ \begin{array}{l}
	\sum_{i \in [n]} \Ex_{x \sim \Ai} \left[ x  \right] = X^A, \\
	%
	\sum_{i \in [n]} \Ex_{x \sim \Bi} \left[ x  \right] = X^B.
	\end{array} \right.
	\label{eq:system_Ex}
\end{align}
By defining the sets $\Iplus:= \braces*{j: p_j \ge 0, {\gB > \frac{p_j}{q_j w_j }} }$, \mbox{$\Iminus := \braces*{j: p_j < 0, {\gA > \frac{-p_j}{w_j }} }$} and the term \mbox{$\hi := \min \{ q_i w_i \gB, w_i \gA + p_i \}$}, and computing the expected values of $\Ai$ and $\Bi$ for $i \in [n]$ (see the details in \ref{sec:appen_proof_OUD}), we can rewrite System~\eqref{eq:system_Ex} as:
\begin{align}
	\left\{ \begin{array}{l}
	g^A (\gA, \gB) = 0, \\
	%
	g^B (\gA,\gB) = 0, 
	\end{array} \right.
	\label{eq:system_f}
\end{align}
%
where $g^A, g^B: \mathbb{R}^2 \rightarrow \mathbb{R}$ are the following functions (for each given instance of the $\FCBn$~game):
% 	\begin{align}
% 	g^A \left(\gA,\gB \right)   &= \frac{1}{X^B} \left[\sum_{i  \in  I^+_2 (\gA,\gB)}\frac{ \left(q_i {w_i} \gB \right)^2 \!-\! \left( {p_i}\right)^2 }{2 q_i w_i } \!+\!   \sum_{i \in I^+_3(\gA,\gB)} \frac{ \left({w_i \gA} \!+\! {p_i}\right)^2 \!-\! \left( {p_i} \right)^2 }{2 q_i w_i} \right] \nonumber \\
% 	& \hspace{3cm} \!+\! \frac{1}{X^B} \left[\sum_{i \in I^-_2(\gA,\gB)}\frac{ \left( {w_i \gA} \!+\! {p_i} \right)^2 }{2 q_i w_i}  \!+\! \sum_{i \in I^-_3(\gA,\gB)}\frac{ \left(q_i {w_i} \gB\right)^2}{2  q_i w_i} \right],  \label{eq:fA}\\
% 	%
% 	\text{ and }	g^B \left(\gA,\gB \right)  &=  \frac{1}{X^A} \left[ \sum_{i \in I^+_2(\gA,\gB)}\frac{ \left({q_i w_i \gB} - p_i \right)^2 }{2 q_i w_i} +   \sum_{i \in I^+_3(\gA,\gB)} \frac{ \left( {w_i} \gA  \right)^2 }{2 q_i w_i} \right]  \nonumber \\
% 	& \hspace{1cm} + \frac{1}{X^A} \left[ \sum_{i \in I^-_2(\gA,\gB)}\frac{ \left(  {w_i} \gA  \right)^2 - p_i^2  }{2 q_i w_i}  + \sum_{i \in I^-_3(\gA,\gB)}\frac{ \left( {q_i w_i \gB}  - p_i \right)^2 - p_i^2}{2 q_i w_i} \right].
% 	\label{eq:fB}
% 	%
% 	\end{align}
\begin{subequations}
    \begin{align}
    	g^A (\gA,\gB )   &\!=\!   \sum \nolimits_{i  \in  \Iplus} \frac{ \bracks*{\hi}^2 \!-\!  {p_i}^2 }{2 q_i w_i } + \sum\nolimits_{i  \in  \Iminus} \frac{ \bracks*{\hi}^2 }{2 q_i w_i} - X^B \gA, \label{eq:fA} \\
    	%
    	g^B (\gA,\gB)   &\!=\!   \sum\nolimits_{i  \in  \Iplus} \frac{ \left[\hi \!-\! p_i\right]^2}{2 q_i w_i } \!+\!  \sum\nolimits_{i  \in  \Iminus} \frac{ \left[ \hi \!-\!p_i \right]^2 \!-\! p_i^2 }{2 q_i w_i}  \!-\! X^A \gB. \label{eq:fB}
    	%
    \end{align}
\end{subequations}
%
%
With these definitions, we can state our main result as the following theorem:
\begin{theorem} \label{theo:OUDs}
    For any game $\FCBn$,
        \begin{itemize}
            \item[$(i)$] There exists a positive solution $\kappa = (\gA, \gB) \in \mathbb{R}^2_{>0}$ of System~\eqref{eq:system_f}.
            %
            \item[$(ii)$] For any positive solution \mbox{$\kappa = (\gA, \gB)\! \in \! \mathbb{R}^2_{>0}$} of System~\eqref{eq:system_f}, the corresponding set of distributions \mbox{$\left\{\Ai,\Bi, i \in [n] \right\}$} from \cref{def:OptDis_GRCBC} is a set of optimal univariate distributions of~$\FCBn$.
        \end{itemize}
\end{theorem}
%
\cref{theo:OUDs} serves as a core result for other analyses in this paper; it is interesting and important in several aspects. First, it shows that in any instance of the $\FCB$ game, there always exists a set of OUDs with the form given in \cref{def:OptDis_GRCBC}. Second, by comparing these OUDs of the $\FCB$ game with that of the classical Colonel Blotto game (see \eg results from \cite{kovenock2020generalizations}), we can see how the pre-allocations and the asymmetric effectiveness affect players' allocations at equilibrium; we will return to this point in \cref{sec:NumExp} with more discussions. Moreover, as candidates for marginals of the equilibrium of the $\FCB$ game (in cases where it exists), the construction of such OUDs allows us to deduce a variety of corollary results concerning equilibria and approximate equilibria of $\FCB$ and $\FGL$ games (we present and discuss them in \cref{sec:Corollary_results} and~\cref{sec:heuristic}). 

We give a detailed proof of \cref{theo:OUDs} in \ref{sec:appen_proof_OUD} and only discuss its main intuition here. First, we can prove Result~$(ii)$ of \cref{theo:OUDs} by simply checking the three conditions of \cref{def:OUD} defining the OUDs of the $\FCB$ game: it is trivial that for $\kappa \in \mathbb{R}^2_{>0}$, the supports of $\Ai, \Bi, \forall i \in [n]$ are subsets of $\Rpos$ (thus, they satisfy Condition~\ref{condi:OUD1}); moreover, if \mbox{$\kappa=(\gA,\gB) \in \R^{2}_{>0}$} is a solution of System~\eqref{eq:system_f}, then it is a solution of System~\eqref{eq:system_Ex} and trivially, $\Ai, \Bi, \forall i \in [n]$ satisfy Condition~\ref{condi:OUD2};\footnote{Note that due to the ``use-it-or-lose-it" rule of the $\FCB$ game, among the existing equilibria (if any), there exists at least one equilibrium in which players use all their resources, thus we only need to consider the equality case of Condition~\ref{condi:OUD2}.} finally, we can check that for each configuration of $w_i, p_i, q_i, \gA, \gB$ (given that $\gA, \gB >0$), the distributions $\Ai, \Bi$ form the equilibrium of the corresponding $\FAPA$ game; thus \mbox{$\Ai,\Bi, i \in [n]$} satisfy Condition~\ref{condi:OUD3}.




On the other hand, proving Result~$(i)$ of \cref{theo:OUDs} is a challenging problem in itself: $g^A$ and $g^B$ are not simply quadratic functions of $\gA$ and $\gB$ since these variables also appear in the conditions of the involved summations. Note that the particular instance of System~\eqref{eq:system_f} where $p_i=0, q_i =1, \forall i \in [n]$ coincides with a system of equations considered in \cite{kovenock2020generalizations} for the case of the classical Colonel Blotto game (without favoritism). Proving the existence of positive solutions of this system \emph{in this particular case} can be reduced to showing the existence of positive solutions of a real-valued 1-dimensional function (with a single variable $\lambda = \gA/\gB$) which can be done by using the intermediate value theorem (see \cite{kovenock2020generalizations}). \emph{In the general case of the $\FCB$ game and System~\eqref{eq:system_f}}, this approach \emph{cannot} be applied due to the involvement of arbitrary parameters $p_i, q_i, i \in [n]$. Alternatively, one can see our problem as proving the existence of a fixed-point in $\R^2_{>0}$ of the function \mbox{$F:\mathbb{R}^2 \rightarrow \mathbb{R}^2$} such that $F \parens*{\gA,\gB} = \parens*{g^A \parens*{\gA,\gB}/X^B + \gA, g^B \parens*{\gA,\gB}/X^A + \gB}$. This direction is also challenging since the particular formulations of $g^A$ and $g^B$ (thus, of $F$) does not allow us to use well-known tools such as Brouwer's fixed-point theorem \cite{brouwer1911abbildung} and/or Poincaré-Miranda theorem \cite{kulpa1997poincare}. 

%Alternatively, one can convert the problem of proving the existence of a positive solution of System~\eqref{eq:system_f} to the following problem: proving the existence of a fixed-point in $\R^2_{>0}$ of the function \mbox{$F:\mathbb{R}^2 \rightarrow \mathbb{R}^2$} such that $F \parens*{\gA,\gB} = \parens*{g^A \parens*{\gA,\gB}/X^B + \gA, g^B \parens*{\gA,\gB}/X^A + \gB}$. This direction is also challenging since the particular formulations of $g^A$ and $g^B$ (thus, of $F$) prevent one to justify sufficient conditions of well-known tools such as Brouwer's fixed point theorem and/or Poincaré-Miranda theorem. 



Instead of the approaches discussed above, in this work, we prove Result~${(i)}$ of \cref{theo:OUDs} via the following equivalent formulation: \emph{proving the existence of a {positive zero}, \ie the existence of a point $(a,b) \in \R^2$ such that $G(a,b)=(0,0)$, of the $G:\R^2 \rightarrow\R^2$} defined as follows:
%
%
\begin{align}
    % G \colon& \phantom{+++}\R^2 \longrightarrow\R^2 \nonumber \\
    &G\parens{\gA,\gB} = \parens*{ g^A \parens{\gA,\gB} , g^B \parens{\gA,\gB}} \in \R^2, \forall (\gA, \gB) \in \R^2. \label{eq:G_func}
\end{align}
%
Note also that although $(0,0)$ is a trivial solution of System~\eqref{eq:system_f} (\ie it is a zero of $G$), we can only construct $\Ai, \Bi$ (as in \cref{def:OptDis_GRCBC}) from solutions whose coordinates are \emph{strictly} positive (\ie only from positive zeros of $G$). In this proof, we work with the notion of \emph{winding numbers} which is intuitively defined as follows: the winding number, denoted $\W \parens*{\curve,y}$, of a parametric (2-dimensional) closed curve $\curve$ around a point $y \in \R^2$ is the number of times that $\curve$ travels counterclockwise around $y$ (see formal definitions of parametric curves, winding numbers and other related notions in \ref{sec:appen_winding}). This notion allows an important result as follows:\footnote{See \cite{chinn1966first} for a more general statement of \cref{lem:wind}. It is also considered in the literature as a variant of the \emph{main theorem of connectedness} in topology (see e.g., Theorem 12.N in \cite{viro2008elementary}).} %
\begin{lemma} \label{lem:wind}
    If $G$ is a continuous mapping, for any set $D \subset \R^2$ which is topologically equivalent to a disk such that $\W(\curve, (0,0)) \neq 0$ where $\curve$ is the $G$-image of the boundary of $D$, then $(0,0) \in G(D)$.
\end{lemma}
%
Our proof proceeds by crafting a tailored set $D \subset \R^2{>0}$ such that the function $G$ from \eqref{eq:G_func} satisfies all sufficient conditions of \cref{lem:wind};\footnote{It is trivial that $g^A( \cdot , \gB), g^A( \gA , \cdot) $ and $g^B( \cdot , \gB), g^B( \gA , \cdot) $ are all continuous and monotone functions in $\mathbb{R}_{>0}$; therefore, from Proposition 1 of \cite{kruse1969joint}, $g^A(\gA, \gB)$ and $g^B(\gA,\gB) $ are continuous functions in~$R^2_{>0}$.} then, we conclude that $G$ has a zero in $D$ and Result~$(ii)$ of \cref{theo:OUDs} follows. 
% \footnote{More precisely, we choose $D \subset \R^2_{>0}$ to be the rectangle (including its interior) whose vertices are $(\eps,\eps), (L,\eps), (L,L)$ and $(\eps,L)$ where $\varepsilon>0$ is a infinitesimally small number and $L$ is a large number (see \ref{sec:appen_proof_OUD} for more details)}
%
Note that finding such a set $D$ and quantifying the involved winding number are non-trivial due to the complexity in the expressions of $g^A$ and $g^B$. We illustrate \cref{lem:wind} and how the proof of Result~$(ii)$ of \cref{theo:OUDs} proceeds in a particular instance of $\FCB$ in \cref{ex:example_1234}.
% We also give an illustration of \cref{lem:wind} and how the proof of Result~$(ii)$ of \cref{theo:OUDs} proceeds in a particular instance of $\FCB$ in \cref{ex:example_1234} in~\ref{appen:heuristic}.
%
\begin{example}\label{ex:example_1234}
	\emph{Consider a game $\FCBn$ with $n = 4$, $X^A=4, X^B=4$, \mbox{$w_1=w_3 =1$}, $w_2 = w_4 =2$, $p_1 = p_2 =1$, \mbox{$p_3 = p_4 =-1$},  $q_i =1, \forall i$. We illustrate in \cref{fig:example_1234} the values of the function $G:\mathbb{R}^2 \rightarrow \mathbb{R}^2$ corresponding to this game. \cref{fig:example_1234}(a) represents the output plane where each point is mapped with a color; e.g., if a point has the color blue, we know that both coordinates of this point are positive. \cref{fig:example_1234}(b) presents the input plane. Function $G$ maps each point in this input plane with a point in the output plane. Then, in \cref{fig:example_1234}(b), we colorize each point in the input plane with the corresponding color of its output (colors are chosen according to \cref{fig:example_1234}(a)). 
% 	For example, in \cref{fig:example_1234}(b), for $\gA \ge 2$ and $\gB \le 1$ (corresponding to the region of green points), by looking up the output plane and find the position of green points, we know that $F(\gA,\gB)$ has a negative $x$-coordinate and a positive $y$-coordinate.
	 Solving \eqref{eq:system_f} in this case, we see that $(2,2)$ is the unique zero of $G$. We observe that in \cref{fig:example_1234}(b), when one choose a disk containing $(2,2)$, its boundary passes through all colors, which indicates that the $G$-image of its boundary goes around the origin $(0,0)$ of the output plane. This is confirmed by \cref{fig:example_1234}(c) showing the $G$-image of a rectangle $D$ having the vertices $(1,1)$, $(1, 4)$, $(4, 4)$, $(4, 1)$ (thus, it contains $(2,2)$); we observe that $G(\partial D)$, which is the blue curve, travels 1 time around $(0,0)$, thus $\W(G(D),(0,0)) \neq 0$.}
% 	{On the other hand, with inputs $\delta =10^{-6}$, our approximation algorithm (initialized with rectangle $D$) outputs the point $(\tgA, \tgB) = (1.9999995, 1.9999995)$ and we can confirm that $G(\tgA, \tgB) = (6.80 \times 10^{-7}, 6.80510 \times 10^{-7})$ (i.e., the error is smaller than~$\delta$). Finally, by listing out all possible combination of indices sets (note again that this is inefficient), we indeed find that $(2,2)$ is an exact zero of $F$ (moreover, it is~unique).}
\end{example}
	


\begin{figure*}[htb!]%
\scriptsize 
		\centering
		\subfloat[][\scriptsize Output plane as a heatmap to be used as reference]{{\includegraphics[height=0.16\textwidth]{Figures/outputcolor.png} }}%
		\qquad \qquad
		\subfloat[][ \scriptsize Input plane with the colors of the values of function $G$]{
			\begin{tikzpicture}
			\node (img){\includegraphics[height=0.14\textwidth]{Figures/inputcolor.png}};
			\node[below=of img, node distance=0cm, yshift=1.2cm, xshift = 0.20cm] {\scriptsize$\gA$};
			\node[left=of img, node distance=-0.2cm, anchor=center,yshift=-0cm,xshift = 0.9cm] {\scriptsize$\gB$};
			\end{tikzpicture}	
		}% 
		\qquad \qquad
		\subfloat[][\scriptsize The image via function $G$ of the rectangle~$D$]{{\includegraphics[height=0.16\textwidth]{Figures/output_curve.png} }}%
		\caption[]{Illustration of the function $G$ on an instance of $\FCBn$ (\cref{ex:example_1234}).}%
		\label{fig:example_1234}%
\end{figure*}






To complete this section, we compute the players' payoffs in the $\FCB$ game in the case where their allocations follow the proposed OUDs. Recall the notation of the indices sets defined in \cref{tab:Opt_Uni_GRCBC}, we have the following proposition (its proof is given in \ref{sec:appen_proof_payoffEQ}):
%
%
\begin{proposition}\label{propo:payoffEQ}
Given a game $\FCBn$ and $\kappa = \parens*{\gA, \gB} \in \R^2_{>0}$, if Players A and B play strategies such that the marginal distributions corresponding to battlefield $i \in [n]$ are $\Ai$ and $\Bi$ respectively, then their payoffs are:
%
\begin{subequations}
    \begin{align}
    	\Pi^A_{\FCBn} & = 	\sum \limits_{i \in I^+_1(\gA,\gB)} {\left[w_i \mathbb{I}_{\{p_i > 0\}} + \alpha w_i \mathbb{I}_{\{p_i =0\}} \right]} \! + \! \sum \limits_{i \in I^+_2(\gA,\gB)} {\left[ w_i \left(1 \!-\! \frac{q_i \gB}{\gA} \!+\! \frac{p_i}{w_i \gA} \right)  \!+\! \frac{(q_i w_i \gB \!-\! p_i )^2}{2 w_i \gA q_i \gB} \right]} \nonumber \\
    	%
    	& \hspace{4mm} +\!  \sum \limits_{i \in I^+_3(\gA,\gB)} \left[ \frac{w_i \gA}{2 q_i \gB} \right] \!+\! \sum \limits_{i \in I^-_2(\gA,\gB)} \left[ \frac{w_i \gA}{2 q_i \gB} \!-\! \frac{p_i ^2}{2 w_i \gA q_i \gB} \right] \!+\!  \sum \limits_{i \in I^-_3 (\gA,\gB)} \left[w_i \!-\! \frac{q_i \gB w_i }{2\gA} \right] \label{eq:payoff_A_GL},\\
    	%
    	%
        \Pi^B_{\FCBn} & = \sum_{i \in [n]} w_i -  	\Pi^A_{\FCBn}. \label{eq:payoff_B_GL}		
    \end{align}
\end{subequations}
\end{proposition}
%

If there exists an equilibrium of the game $\FCBn$ whose marginals are $\Ai, \Bi, i \in [n]$, then \eqref{eq:payoff_A_GL} and \eqref{eq:payoff_B_GL} are formulations of the equilibrium payoffs in this game. Observe, however, that as $p_i$ and $q_i$ (and $w_i$) change, System~\eqref{eq:system_f} also changes; thus, its solutions also vary and the configuration of the corresponding indices sets change. Therefore, the relationship between the favoritism parameters and the payoffs induced by the corresponding OUDs is \emph{not} easily deducible from \eqref{eq:payoff_A_GL}-\eqref{eq:payoff_B_GL}. We delay our discussion on this to \cref{sec:NumExp} where we present results from numerical~experiments.













%
%
%---------------------------










==> EC ArXiV - Upload/Sections/game_formu.tex <==
%!TEX root = ../main.tex


In this section, we define the Colonel Blotto game with favoritism ($\FCB$), and two related models: the General Lotto game with favoritism ($\FGL$) and the all-pay auction with favoritism ($\FAPA$).%

	
%%%%%%%%%%%%%%    
\subsection{Colonel Blotto and General Lotto Games with Favoritism}
\label{sec:FormCB}
%
The Colonel Blotto game with favoritism (\FCB game) is a one-shot complete-information game between two Players A and B. Each player has a fixed \emph{budget} of resources, denoted $X^A$ and $X^B$ respectively; without loss of generality, we assume that \mbox{$0< X^A \le X^B$}. There are $n$ battlefields ($n \ge 3$). Each battlefield $i \in [n]$ has a value $w_i>0$ and is embedded with two additional parameters: $p_i \in \mathbb{R}$ and $q_i>0$. Knowing these parameters, players compete over the $n$ battlefield by simultaneously allocating their resources. The summation of resources that a player allocates to the battlefields cannot exceed her budget; i.e., the {pure strategy} set of Player ${\play} \in \left\{ A, B \right\}$ is $S^{\play} = \left\{ \boldsymbol{x}^{\play} \in \mathbb{R}_ {\ge 0} ^n: \sum\nolimits_{i = 1}^n {x_i^{\play} \le {X^{\play}}} \right\}$. If Players A and B respectively allocate $x^A_i$ and $x^B_i$ to battlefield $i$, the winner in this battlefield is determined by the following rule: if $x^A_i > q_i x^B_i -p_i$, Player A wins and gains the value $w_i$; reversely, if $x^A_i < q_i x^B_i -p_i$, Player B wins and gains $w_i$; finally, if a tie occurs, i.e., $x^A_i = q_i x^B_i -p_i$, Player A gains $\alpha w_i$ and Player B gains $(1-\alpha) w_i$, where $\alpha \in [0,1]$ is a given parameter.\footnote{We call $\alpha$ the tie-breaking parameter. It can be understood as if we randomly break the tie such that Player A wins battlefield $i$ with probability $\alpha$ while Player B wins it with probability $(1-\alpha)$. This includes all the tie-breaking rules considered in classical CB games found in the literature.} The payoff of each player in the game is the summation of gains they obtain from all the battlefields. Formally, we have the following definition.
%\footnote{Henceforth, we address the inequalities $\sum\nolimits_{i = 1}^n {x_i^{\play} \le {X^{\play}}}$ for $\play \in \{A,B\}$ as the budget constraints.}


\begin{definition}[The \FCB game]
\label{def:FCB}
The Colonel Blotto game with favoritism (with $n$ battlefields), denoted $\FCBn$, is the game with the description above; in particular,  when players A and B play the pure strategies \mbox{$\boldsymbol{x}^A = \parens*{x^A_i}_{i \in [n]}\! \in \! S^A$} and \mbox{$\boldsymbol{x}^B  = \parens*{x^B_i}_{i \in [n]} \in S^B $} respectively, their payoffs are defined as:
\begin{equation*}
    \mathrm{\Pi}_{\FCBn}^A \left( \boldsymbol{x}^A, \boldsymbol{x}^B \right) = \sum \limits_{i \in [n]} {w_i   \be \left( x^A_i, q_i x^B_i \!- \!p_i \right)  } \textrm{ and } \mathrm{\Pi}_{\FCBn}^B \left( \boldsymbol{x}^A, \boldsymbol{x}^B  \right) =\sum \limits_{i \in [n]} {w_i   \left[ 1\!-\! \be \left( x^A_i, q_i x^B_i\! - \!p_i \right) \right]  }.
\end{equation*}
Here, $\be: \mathbb{R}^2_{\ge 0} \rightarrow [0,1]$, termed as the Blotto function, is defined as follows: $\be\left( {x,y} \right)=1$ if $x>y$, $\be\left( {x,y} \right)=\alpha$ if $x=y$ and $\be\left( {x,y} \right)=0$ if $x<y$. 
  %	
%   	\begin{equation}
% 		\be\left( {x,y} \right) = \left\{ \begin{array}{l}
% 		1 \text{ , if } x >y\\
% 		\alpha \text{ , if } x =y \\
% 		0 \text{ , if } x < y
% 		\end{array} \right. . \label{eq:betafunction}
%     \end{equation}  
\end{definition}
	
	
	
A \emph{mixed strategy} of a player, say $\play \in \braces*{A,B}$, in $\FCBn$ is an $n$-variate distribution such that any pure strategy drawn from it is an $n$-tuple satisfying the corresponding budget constraint of player~$\play$. We reuse the notations $\mathrm{\Pi}_{\FCBn}^A \left(\sigma_A, \sigma_B \right)$ and $\mathrm{\Pi}_{\FCBn}^B \left(\sigma_A, \sigma_B \right)$ to denote the payoffs of Players A and B when they play the mixed strategies $\sigma_A$ and~$\sigma_B$ respectively. Note that to lighten the notation $\FCBn$, we include only the subscript $n$ (the number of battlefields) and omit other parameters involved in the definition of the game (including $X^A, X^B, \alpha, w_i, p_i, q_i, \forall i \in [n]$). 

The game $\FCBn$ extends the classical Colonel Blotto game by including the favoritism that a player may have in battlefield $i$ through the parameters $p_i$ and $q_i$; which can be interpreted as~follows: 
\begin{trivlist}
	\item[$(i)$] $p_i$ represents the difference between pre-allocations that players have at battlefield $i$ before the game begins (note that pre-allocations are not included in the players' budget $X^A$ and $X^B$). If $p_i >0$, Player A's pre-allocation at battlefield $i$ is larger; if $p_i<0$, Player B has a larger pre-allocation.
	%
	\item[$(ii)$] $q_i$ represents the asymmetry in the effectiveness of players' resources (\emph{not} including the pre-allocations). Specifically, in battlefield $i$, each unit of Player~B's resource is worth $q_i$ units of Player A's resource. If $0< q_i < 1$, Player A's resource is more effective than that of Player B; reversely, if $  q_i > 1$, Player B's resource is more effective. %
\end{trivlist}
%
%As far as we know, our model of the \FCB game is novel. It is also more general than other versions of CB games considered in the literature (except the generalized CB game considered in \cite{kovenock2015}); indeed, 
Note that if $p_i =0$ and $q_i = 1, \forall i \in [n]$, the game $\FCBn$ coincides with the classical CB game. Unlike many works in the literature on classical CB game, in the $\FCBn$ game defined above, we do not make assumptions on the symmetry in players' budgets or on the homogeneity of the battlefields'~values. 


For the sake of conciseness, in the remainder, we consider \FCB under the following assumptions:
%

\begin{assumption} \label{assum:1}
    $\sum_{i \in [n]} {\parens*{q_i X^B - p_i}} \ge X^A$ and $\sum_{i \in [n]} { \parens*{X^A + p_i} /q_i } \ge X^B $. 
\end{assumption}
%
\begin{assumption}\label{assum:2}
    For any $i \in [n]$, $\parens*{q_i X^B - p_i} \ge 0$ and $\parens*{X^A + p_i} /q_i \ge 0$.
\end{assumption}
		%
These assumptions are used simply to exclude trivial cases where one player has too strong favoritism in one (or all) battlefields. Indeed, if \cref{assum:1} is violated, there exists trivial pure equilibria.\footnote{If $\sum_{i \in [n]} {\parens*{q_i X^B - p_i}} < X^A$, by allocating $q_i X^B - p_i + \varepsilon $ to battlefield $i$ ($\varepsilon$ is an arbitrarily small number), Player A guarantees to win all battlefields regardless of Player B' allocations. If $\sum_{i \in [n]} { \parens*{X^A + p_i} /q_i } < X^B $, by allocating $\parens*{X^A + p_i} /q_i + \varepsilon$ to battlefield $i$, Player B guarantees to win all battlefields.} On the other hand, if in battlefield $i^* \in [n]$, $\parens*{q_{i^*} X^B - p_{i^*}} < 0$ (resp. $\parens*{X^A + p_{i^*}} /q_{i^*} < 0$), then by allocating 0, Player A (resp. Player B) guarantees to win this battlefield regardless of her opponent's allocation. Therefore, if $\FCBn$ has an battlefield $i^*$ violating \cref{assum:2}, an equilibrium of $\FCBn$ is simply the strategies where both players allocate 0 to battlefield $i^*$ and play an equilibrium of the game $\mathcal{CB}^F_{n-1}$ having the same setting as $\FCBn$ but excluding battlefield $i^*$. Note that analogous assumptions (when $p_i = 0$ and $q_i = 1, \forall i$) are found in other works considering the classical CB game (see \eg \cite{roberson2006} and Figure 1 in \cite{kovenock2020generalizations}).



Next, similar to the definition of the General Lotto game obtained from relaxing the classical CB game, for each instance of the \FCB game, we define an instance of the General Lotto with favoritism ($\FGL$) where the budget constraint is requested to hold only in expectation. Formally:
\begin{definition}[The \FGL game]
    \label{def:FGL}
    The General Lotto game with favoritism (with $n$ battlefields), denoted $\FGLn$, is the game with the same setting and parameters as the $\FCBn$ game, but where a mixed strategy of Player $\play \in \{A,B\}$ in $\FGLn$ is an $n$-variate distribution with marginal distributions $(F^{\play}_i)_{i \in [n]}$ such that \mbox{$\sum_{i \in [n]} {\Ex_{x_i \sim F^{\play}_i }[ x_i ] } \le X^{\play}$}. 
    %In particular, when players play the mixed strategies $\sigma^A = \left(F^A_i \right)_{i \in [n]}$ and \mbox{$\sigma^B = \left(F^B_i \right)_{i \in [n]}$}, their expected payoffs in $\FGLn$ are $\mathrm{\Pi}_{\FGLn}^A \left( \sigma^A, \sigma^B \right) = \sum_{i \in [n]} \mathop{\Ex} \limits_{\substack{ x^A_i \sim F^A_i \\ x^B_i \sim F^B_i} } {w_i  \cdot \be \left( x^A_i, q_i x^B_i - p_i \right)  }$ and $\mathrm{\Pi}_{\FGLn}^B \left( \sigma^A, \sigma^B \right) = \sum_{i \in [n]} \mathop{\Ex} \limits_{\substack{ x^A_i \sim F^A_i \\ x^B_i \sim F^B_i} } {w_i  \cdot [1 - \be \left( x^A_i, q_i x^B_i - p_i \right) ] }$.
\end{definition}

	
	
	
	
We finally define the notion of Optimal Univariate Distributions in the $\FCB$ game. This notion is of great importance in studying equilibria of the \FCB game since intuitively, they are the candidates for the marginals of the equilibria. Formally:
\begin{definition}[Optimal Univariate Distributions (OUDs)] \label{def:OUD}
    $\left\{F^A_i, F^B_i: i \in [n] \right\}$ is a set of \emph{OUDs} of the game $\FCBn$ if the following conditions are satisfied:
    \begin{enumerate}[label=(C.\arabic*),ref=\textit{(C.\arabic*)}]
        \item  the supports of $F^A_i, F^B_i$ are subset of $\mathbb{R}_{\ge 0}$, \label{condi:OUD1}
        %
        %
        \item \mbox{$\sum_{i \in [n]} {\Ex_{x_i \sim F^\play_i }[ x_i ] } \le X^{\play}$}, $\play \in \{A,B\}$, \label{condi:OUD2}
        %
        \item if Player $\play$ draws her allocation to battlefield $i$ from $F^\play_i$, $\forall i \in [n]$, Player $-\play$ has no pure strategy inducing a better payoff than when she draws her allocation to battlefield $i$ from $F^{-\play}_i$, $\forall i \in [n]$.\label{condi:OUD3}
    \end{enumerate}
\end{definition}
%\textbf{add a small intuition on those?}

	
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{All-pay Auctions with Favoritism}
\label{sec:FormAPA}
%
All-pay auctions with favoritism ($\FAPA$) have been studied in the literature under different sets of assumptions (see \cref{sec:Intro}). For the sake of coherence, in this section, we re-define the formulation of the \FAPA game using our notation as follows:

In the \FAPA game, two players, A and B, compete for a common item that is evaluated by each player with a value, denoted $u^A$ and $u^B$ respectively ($u^A, u^B > 0$).\footnote{The case where either $u^A =0$ or $u^B =0$ is trivial (there exist trivial pure equilibria) and thus, is omitted.} The item is embedded with two additional parameters: $p \in \mathbb{R}$ and $q>0$. Players simultaneously submit their \emph{bids} $x^A, x^B \ge 0$ (unlike in the $\FCB$ game, players can bid as large as they want in $\FAPA$). If $x^A > q x^B - p$, Player A wins the item and gains the value $u^A$; if $x^A < q x^B - p$, Player B wins and gains the value $u^B$; and in case of a tie, i.e., $x^A = q x^B -p$, Player A gains $\alpha u^A$ and Player B gains $(1-\alpha) u^B$ ($\alpha \in [0,1]$). Finally, \emph{both players} pay their bids. % that they submitted. % (regardless of the winner). Formally, we have the following~definition:
\begin{definition}[The \FAPA game] \label{def:APA-F}
	\emph{\FAPA} is the game with the above description; in particular, when the players A and B bid $x^A$ and $x^B$ respectively, their payoffs are \mbox{$\mathrm{\Pi}^A_{\FAPA} \left( x^A, x^B \right) \!= \!u^A \be \left( x^A, q x^B \!-\! p \right) \!-\! x^A$} and \mbox{$\mathrm{\Pi}^B_{\FAPA} \left( x^A, x^B \right) \!= \!u^B [1-\be \left( x^A, q x^B \!-\! p \right)] \!-\! x^B$}. Here, the function $\be$ is defined in \cref{def:FCB}.
\end{definition}
%
%
The formulation of the \FAPA game presented above differs from classical all-pay auctions by the parameters $p$ and $q$. If $p>0$, Player A has an \emph{additive advantage} in competing to win the item and if $p<0$, Player B has this favoritism; likewise, when $0<q<1$, Player A has a \emph{multiplicative favoritism} to compete for the item and when $q>1$, it is in favor of Player B. Our formulation of \FAPA is more general than the models (with two players) considered by previous works in the literature. If $p=0$, $q=1$ and $\alpha=1/2$, the $\FAPA$ game coincides to the classic two-bidder (first-price) all-pay auction (e.g., in \cite{baye1994,hillman1989}). If $u^A = u^B$, $\alpha = 1/2$, $p>0$ and $0<q \le 1$ (i.e., Player A has both advantages), $\FAPA$ coincides with the framework of all-pay contests with incumbency advantages considered in \cite{konrad2002investment}. Moreover, we also define \FAPA with a generalization of the tie-breaking rule (with the parameter $\alpha$ involving in the function $\be$) covering other tie-breaking rules considered in previous works. Finally, our definition of $\FAPA$ and its equilibria characterization (see \cref{sec:EquiAPA}) can also be extended to cases involving more than two players/bidders; in this work, we only analyze the two-player $\FAPA$ since it relates directly to the \FCB game, which is our main~focus.

	
	
	
	
	
	
	
	
	
	
	
	

	
	
	

==> EC ArXiV - Upload/Sections/introduction.tex <==
%!TEX root = ../main.tex
	
	
The \emph{Colonel Blotto game}, first introduced by \cite{borel1921}, is a famous resource allocation games. Two players A and B compete over $n$ battlefields by simultaneously distributing resources such that the sum of each player's allocations does not exceed her budget (the so-called \emph{budget constraint}). Each battlefield has a certain value. In each battlefield, the player who has the higher allocation wins and gains the whole battlefield's value while the other player gains zero; this is the \emph{winner-determination rule}. The total payoff of each player is the sum of gains from all the battlefields. 
	
The Colonel Blotto game captures a large range of practical situations. Its original application is \emph{military logistic} \cite{gross1950,grosswagner}, where resources correspond to soldiers, equipment or weapons; but it is now also used to model \emph{security problems} where battlefields are security targets and resources are security forces or effort \cite{chia2012,schwartz2014}, \emph{political competitions} where players are political parties who distribute their time or money resources to compete over voters or states \cite{kovenock2012,myerson1993incentives,roberson2006}, \emph{competitions in online advertising} \cite{masucci2014,masucci2015}, or \emph{radio-spectrum management systems} \cite{hajimirsaadeghi2017dynamic}.

In many of these applications, however, the winner-determination rule of the Colonel Blotto game is too restrictive to capture practical situations because a player might have an advantage over some battlefields; we refer to this as \emph{favoritism}. There can be two basic types of favoritism:
\begin{trivlist}
    \item[\emph{First},] players may have resources committed to battlefields before the game begins---we refer to them as \emph{pre-allocations}. These pre-allocations then add up to the allocations to determine the winner in each battlefield. In military logistics for instance, before the start of military operations, it is often the case that one side (or both) already installed military forces on some battlefields. Pre-allocations can also be found in R\&D contests, where companies can use the technologies they currently possess to gain advantage while competing to develop new products/technologies. In political contests, it is often the case that voters have an a priori position that may be interpreted as a pre-allocation of the corresponding party (e.g., Californian voters are in majority pro-Democrats). 
    %
    \item[\emph{Second},] the \emph{resources effectiveness} may not be the same for both players, and may vary across battlefields. For example, in airport-surveillance, it often requires several agents to patrol a security target while a single terrorist may suffice for a successful attack. In military logistics, the effectiveness of resources (equipment, soldiers, etc.) may differ amongst players and vary according to the landscapes/features of the battlefields. In R\&D contests, one unit of resources (researchers/machines) of a company often has different strengths and weaknesses than that of other companies.
\end{trivlist}


 %Asymmetric effectiveness can also be found in political contests such as the US presidential election, e.g., resources of the Democratic party is more effective when it is spent in California than in swing states (e.g.,~Virginia).
	
	

	
%Another example is in advertising on social media where marketing campaigns (i.e., players) compete over high-influence social network users (i.e., battlefields) by giving them promotional gifts to convince them to motivate their peers to buy advertised products: users might have biased opinions on products, thus, certain campaigns already have advantages before the beginning of the game.
	

In this work, we propose and analyze an extension of the Colonel Blotto game with a winner-determination rule capturing pre-allocations and asymmetric effectiveness of resources. Specifically, we consider the following rule: in battlefield $i \in \{1,\cdots, n\}$, if the allocations of Players A and B are $x^A$ and $x^B$ respectively, Player A wins if $x^A > q_i \cdot x^B - p_i$ and Player B wins otherwise (we will specify the tie breaking rule below). Here, $p_i \in \mathbb{R}$ and $q_i >0$ are given parameters known to both players that represent pre-allocations and asymmetric effectiveness of resources respectively. We call this game the \emph{Colonel Blotto game with favoritism} and denote it by \FCB throughout the paper. We focus on characterizing and computing Nash equilibria of the \FCB game. 
%. Note that we allow players' budgets to be asymmetric, battlefields' values to be heterogeneous and the tie-breaking rule to be general 
%\emph{The} \FCB \emph{game is our primary focus in this work and the key question in studying this game is how to play strategically to obtain good guarantees on~payoffs}. 


%given parameters $p_i \in \mathbb{R}$ and $q_i >0$, if the allocations of Players A and B are $x^A$ and $x^B$ respectively, then, Player A wins this battlefield if $x^A > q_i \cdot x^B - p_i $ and Player B wins if $x^A < q_i \cdot x^B - p_i$, the winner gains the corresponding value and the loser gains zero.\footnote{If $x^A = q_i \cdot x^B - p_i$, a pre-defined tie-breaking rule will be used to determine players' gains from battlefield~$i$.} Intuitively, the parameter $p_i$ represents the difference between players' pre-allocations while $q_i$ represents the asymmetry between effectiveness of players' resources. We call this game the \emph{Colonel Blotto game with favoritism} (henceforth, \FCB game). Note that unlike most works in the literature studying Colonel Blotto games, we allow players' budgets in \FCB to be asymmetric, battlefields' values to be heterogeneous and the tie-breaking rule to be generalized (see \cref{sec:FormCB} for a formal definition of $\FCB$). \emph{The} \FCB \emph{game is our primary focus in this work and the key question in studying this game is how to play strategically to obtain good guarantees on~payoffs}. 
	
Completely characterizing and computing a Nash equilibrium of the Colonel Blotto game, even without favoritism, is a notoriously challenging problem (see related works below). A standard approach consists in first identifying candidate equilibrium marginal distributions for each battlefield's allocation---called the \emph{optimal univariate distributions}. This is often done by looking for an equivalence to the related problem of all-pay auctions---the game where two bidders secretly bid on a common item and the higher bidder wins the item and gains its value but both players pay their bids. Then, constructing an equilibrium based on these univariate distributions can be done exactly for some particular cases of parameters configurations (see related works below). In cases where this is not possible, an alternative solution is to look for \emph{approximate equilibria} with well-controlled approximation errors \cite{vu2019approximate}. Several works also consider a relaxation of the game with  budget constraints in expectation only---which is called the \emph{General Lotto game}---as a relevant model for certain applications \cite{myerson1993incentives,kovenock2020generalizations}. 
%Besides the Colonel Blotto game (\ie where budget constraints hold with probability 1), the game variant relaxing the budget constraint to hold only in expectation---which is called the \emph{General Lotto game}---also attracts the attention of the literature (see \eg \cite{kovenock2020generalizations,myerson1993incentives}); it can be used to model several practical situations, \eg in politics and R\&D. 
%\footnote{In all-pay auctions, players have no budget but their bids are subtracted from their payoffs.}

In this paper, we analyze the Colonel Blotto game with favoritism by following a similar pattern and make four main contributions as follows: 
\begin{enumerate}
    \item We first consider the model of \emph{all-pay auction with favoritism} ($\FAPA$), where the rule determining the winning bidder is shifted with an additive and a multiplicative parameter. We completely characterize the equilibria in general parameters configurations (with asymmetric items evaluation and no restriction on which bidder has which kind of favoritism). While the \FAPA game was studied in prior works, this result fills a gap in the literature. 
    
%    We study an extension of the all-pay auctions model, called the \emph{all-pay auction with favoritism} ($\FAPA$) where the rule determining the winner among the bidders is shifted with an additive parameter and a multiplicative parameter (similar to that of the \FCB game). We completely characterize the equilibria of this game in general parameters configurations (i.e., bidders have asymmetric evaluation on items and there is no restriction on which bidder has which kind of favoritism). This result fills a gap in the literature on the (two-player) \FAPA. 
    %
    \item We prove the existence of a set of optimal univariate distributions of the \FCB game and give a construction thereof. The main challenge is that it is equivalent to finding a fixed point, but for a complex two-dimensional function for which standard existence results fail to apply. We overcome this obstacle by drawing tools from topology and carefully tailoring them to our particular problem. 
%    Unlike the classical Colonel Blotto game, obtaining this result is challenging since it is equivalent to the problem of finding fixed-points of a two-dimensional function with inevitably complicated algebraic expressions; we overcome this obstacle by drawing tools from topology and carefully tailoring them for the problems in consideration. 
    % To do this, we prove that there exists a positive solution of the system of equations requiring that the aggregate of expected values of the involved distributions (yielding the equilibria of the corresponding $\FAPA$) equal the players' budgets. {Unlike the classical Colonel Blotto game, proving the existence of such solutions (and thus, constructing the corresponding set of optimal univariate distributions of the \FCB game) is a challenging problem in itself.}
    Based on this core result, we deduce the equilibrium of the \FCB game for particular cases for which it is known how to construct joint distributions from the optimal univariate distributions. For other cases we show that, by applying the rescaling technique of \cite{vu2019approximate}, we can obtain an approximate equilibrium of the $\FCB$ game with negligible approximation error when the number of the battlefields is~large. Finally, for any parameter configuration, we immediately obtain the equilibrium of the relaxed \emph{General Lotto game with favoritism} in which one can simply sample independently on each battlefield.
%    Based on this core result, we analyze several known cases of the \FCB game in which it is available to find an equilibrium of the $\FCB$ game by constructing joint distributions from these optimal univariate distributions. We also show that drawing independently from these univariates is an equilibrium of the \emph{General Lotto with favoritism} and that by applying the rescaling scheme of \cite{vu2019approximate}, we can obtain an approximate equilibrium of the $\FCB$ game with negligible approximation errors when the number of the battlefields is~large.
    %
    \item 
We propose an algorithm that efficiently finds an approximation of the proposed optimal univariate distributions with arbitrarily small error. This improves the scalability of our results upon the naive solution for exact computation (which is exponential in the number of battlefields). Our algorithm is based on approximately solving the two-dimensional fixed-point problem by a dichotomy procedure using a generalization of the intermediate value theorem with the notion of winding number of parametric curves. 
    
%We propose an algorithm that efficiently finds an approximation of the proposed optimal univariate distributions with arbitrarily small approximation errors; this improves the scalability of our results to large-scaled problems in practice.\footnote{Direct computation of these optimal univariate distributions, while doable, is not efficient: it requires a running time that is exponential in terms of the number of battlefields.} Our algorithm is based on converting the problem into finding a fixed-point of a function from $\mathbb{R}^{2}$ to $\mathbb{R}^{2}$, then approximately solving it by a dichotomy procedure using a generalization of the intermediate value theorem with the notion of winding numbers of parametric curves. 
    %
    \item We conduct a number of numerical experiments to analyze and illustrate the effect of favoritism in the players' payoffs at equilibrium of the \FCB~game (and of the \FGL game).
\end{enumerate}
%
  


%Finally, we also consider two other game models that is closely related to the \FCB game. First, in the literature, there exists a relaxed version of the Colonel Blotto game, known as the \emph{General Lotto game} (henceforth, General Lotto game), where budget constraints are only required to be satisfied in expectation. This relaxed constraint can be found in several cases of applications and the General Lotto game is useful to study them. More importantly, solutions of the General Lotto game are often used as tools to study the Colonel Blotto game (see e.g., \cite{kovenock2020generalizations,myerson1993incentives}) and \cref{sec:Contri} for more details). In this work, we define and study the \emph{General Lotto game with favoritism} (henceforth, $\FGL$) that is relaxed from the \FCB game. Another model relating to the Colonel Blotto game is the all-pay auction (henceforth, all-pay auctions), its classical version is described as follows: two bidders (i.e., players) secretly decide their bids to compete for a common item; the bidder having the higher bid wins the item and gains its corresponding value; then, both players pay their bids.\footnote{Note that unlike CB (and GL) games, in all-pay auctions, players can bid/allocate as large as they want and their payoffs are subtracted by their bids (i.e., allocations).} all-pay auctions has applications in politics, sports, etc., and it has a long-standing history of being studied (see e.g., \cite{fu2019contests} for a survey). In the literature, it is common to use all-pay auctions as a tool to find Nash equilibria\footnote{Henceforth, we refer to Nash equilibria simply as equilibria.} of CB and General Lotto games (see e.g., \cite{kovenock2020generalizations,roberson2006,schwartz2014}). Motivated by this reason, in this work, we study a special extension of the all-pay auctions model, called the \emph{all-pay auction with favoritism} (henceforth, $\FAPA$) where the rule determining winners among the bidders is shifted with an additive parameter and a multiplicative parameter (similar to that of the \FCB game)---see \cref{sec:Formall-pay auctions} for a formal definition. We aim to characterize the equilibria of the two-player \FAPA in its general setting then use this result to analyze the \FCB and \FGL games. 
	
	


	
	
	
%
%
%%%%%%%%
%%%%%%%%
\paragraph{\textbf{Related Work}}
% \label{sec:Literature}
%
There is a rich literature on characterizing equilibria of the (classical) Colonel Blotto game. The common approach is to look for a set of \emph{optimal univariate distributions} of the game, and then construct $n$-variate joint distributions \emph{whose realizations satisfy the budget constraints} (in other words, their supports are subsets of the (mixed) strategy sets). These joint distributions are equilibria of the game. Constructing such joint distributions, however, is challenging and equilibria are only successfully characterized in several restricted instances: Colonel Blotto games where players have symmetric budgets \cite{borel1938,gross1950,grosswagner,laslier2002,thomas2017,Boix-Adsera20a}, Colonel Blotto games with asymmetric budgets and two battlefields \cite{macdonell2015} or with any number of battlefields but under assumptions on the homogeneity of battlefields' values \cite{roberson2006,schwartz2014}. The Colonel Blotto game still lacks a complete characterization of equilibrium in its generalized parameters configuration, i.e., with asymmetric budgets and heterogeneous battlefields (see \cite{kovenock2012conflicts} for a survey). An extension of the Colonel Blotto game is studied in \cite{kovenock2020generalizations}, where the two players can have different evaluations of the battlefields. The authors find a set of optimal univariate distributions based on a solution of a fixed-point equation, but they can construct the n-variate equilibrium distribution only in restricted settings. Our work follows a similar pattern in spirit, but the fixed-point equation supporting the optimal univariate distributions is different and harder to solve because it is two-dimensional. 


While studying the Colonel Blotto game, many works also consider the corresponding General Lotto game \cite{kovenock2020generalizations,myerson1993incentives}, in which budget constraints are relaxed to hold in expectation. There, an equilibrium can be directly obtained from a set of optimal univariate distributions by independently drawing on each battlefield. In recent work, \cite{vu2019approximate} propose an alternative approach to find solutions of the Colonel Blotto game: it consists of independently drawing on each battlefield and then rescaling to meet the budget constraint with probability one. The authors show that this rescaling strategy (termed independently uniform ($\IU$) strategy) yields an approximate equilibrium with error decreasing with the number of battlefields. %; even in cases where an exact equilibrium cannot be~computed.




The problem of constructing sets of optimal univariate distributions in the Colonel Blotto game can be converted into the problem of searching for an equilibrium of an all-pay auction. The state-of-the-art in characterizing equilibria of all-pay auctions is as follows: equilibria of the (classical) all-pay auctions were completely characterized by \cite{baye1994,hillman1989} in games with any number of~bidders. The all-pay auction with favoritism (also referred to as all-pay auctions with head-starts and handicaps and all-pay auctions with incumbency advantages) was studied by \cite{konrad2002investment} but its equilibria were explicitly characterized only in cases where players assess the item with the same value and where both kinds of favoritism are in favor of one player. Therefore, it still lacks an explicit analysis of equilibria with a general configuration of parameters. Note also that the literature on the \FAPA game (and all-pay auctions) goes beyond the study on their equilibria, see e.g., \cite{fu2006theory,li2012contests,pastine2012incumbency,siegel2009all,siegel2014asymmetric} and surveys by \cite{corchon2007theory,fu2019contests,konrad2009}.
% \footnote{For example, \cite{siegel2009all,siegel2014asymmetric} study a general transformation in winner-determination rule; \cite{fu2006theory,li2012contests,pastine2012incumbency} study the optimal decisions of players in choosing the head-start in a variety of scenarios; \cite{clark2000allocation,kirkegaard2012favoritism,kitahara2010all} focus on the game where item's valuations are incomplete information.}


Our work is the first to introduce the Colonel Blotto game with pre-allocations and asymmetric effectiveness of players' resources. The only exception is the recent work by \cite{chandan2020showing}, where partial results are obtained with pre-allocations only but from a very different perspective: the authors study a three-stage Colonel Blotto game that allows players to pre-allocate their resources; several conditions where pre-allocating is advantageous are indicated and this result is extended to three-player Colonel Blotto games. Note finally that there is also a growing literature on the discrete Colonel Blotto game, where players' allocations must be integers, see \eg \cite{Ahmadinejad16a,Behnezhad19a,Behnezhad17a,behnezhad2018battlefields,hart2008,hortala2012,vu18a,vu2020}; but this literature did not consider favoritism and these results are based on a very different set of techniques in comparison to that of the game models considered in this work.


%There exist works in the literature studying versions of the Colonel Blotto game where players may have pre-allocations in which partial results are obtained but with different perspectives from our work. For example, \cite{chandan2020showing} studies a three-stage Colonel Blotto game that allows players to pre-allocate their resources; several conditions where pre-allocating is advantageous are indicated and this result is extended to three-player Colonel Blotto games. We are not aware of any work considering Colonel Blotto games with asymmetric effectiveness of players' resources. As far as we know, our work is the first to study the extension of the Colonel Blotto game considering cases involving both types of~favoritism (represented by exogenous parameters). 



%Recently, another approach in examining players' behaviors in Colonel Blotto games is proposed, i.e., studying approximate equilibria with well-controlled approximation error. Particularly, \cite{vu2019approximate} proposes a simply-constructed approximate equilibria of the Colonel Blotto game (in its generalized parameters configurations), called the independently uniform strategy (henceforth, $\IU$ strategy),\footnote{A similar scheme is also used in \cite{vu18a} for discrete Colonel Blotto games (where allocations and budgets are indivisible).} that yield a negligible error when the number of battlefields is large. The main idea of the $\IU$ strategy is to let players independently draw allocations from a set of optimal univariate distributions (that are uniform-type distributions) then rescale them to guarantee the budget constrains of the CB~game. 

%\footnote{$\left\{ F^A_i, F^B_i \! :\! i \!\in \! [n] \right\}$ is called a set of \emph{optimal univariate distributions} if when player $\play \in \{A,B\}$ draws her allocation to battlefield $i$ from $F^\play_i$, her budget constraints hold in expectation and if that is the case, it is optimal for player $-\play$ to draw her allocation to battlefields $i$ from $F^{-\play}_i$---see \cref{sec:FormCB} for a formal~definition.}  
%Note that \cite{kovenock2020generalizations} studies a game extension (where players might also have different evaluations on values of battlefields) and shows a method to find a set of optimal univariate distributions, then indicates a sufficient condition\footnote{It requires that if the set of battlefields are partitioned such that two battlefields are in the same partition if they have the same values; then, there exists a sufficient number of battlefields in each partition.} for these optimal univariate distributions to become the marginals of an equilibrium; however, this result only covers a very restricted range of games.

	
	

	
	

	
	
	
	
%In this work, we introduce and formally define the formulation of the Colonel Blotto game with favoritism ($\FCB$). As a preparation for our analyses on $\FCB$, we first study \FAPA and our \textbf{first contribution} is to completely characterize equilibria of this game in general parameters configurations (i.e., players/bidders have asymmetric evaluation on items and there is no restriction on which player/bidder has which kind of favoritism). This result extends the scope of applications and fills in the gaps in the literature of the \FAPA model. Based on the equilibria of $\FAPA$, we construct a set of optimal univariate distributions of the \FCB game, these optimal univariate distributions constitute an equilibrium of the corresponding \FGL game---this is our \textbf{second contribution}. These results are obtained under a sufficient condition that there exist positive solutions of a particular system of equations (requiring that the aggregate of expected values of the optimal univariate distributions does not exceed players' budgets). It remains an open question to theoretically prove that this sufficient condition holds for any \FCB game; moreover, a direct computation of solutions (if they exist) of this system---while doable---is still inefficient (having a running time in an exponential order in terms of the number of battlefields). Addressing this problem, our \textbf{third contribution} is to propose a heuristic procedure that efficiently find an approximate solution of the aforementioned system with arbitrarily small approximation errors. Then, we show that the $\IU$ strategy rescaling the optimal univariate distributions corresponding to the approximate solution obtained from our heuristic procedure is an approximation equilibrium of the $\FCB$ game---this is our \textbf{fourth contribution}. We also show that the involved approximation error of this IU strategy is negligible for games with a large number of battlefields, which often found in practice. These results give a practical way to analyze players' behaviours in applications of the $\FCB$ game (and $\FGL$ game). Finally, we conduct several numerical experiments to illustrate the obtained theoretical~results. 
	
	
	
	
% 	\vspace{-3mm}
%%%%%%%%%%%%
\paragraph{\textbf{Notation}}
% REMEMBER TO REWRITE THIS LEST IT COLLAPSE WITH OTHER PAPERS:
Throughout the paper, we use bold symbols (e.g., $\boldsymbol{x}$) to denote vectors and subscript indices to denote its elements (e.g., $\boldsymbol{x} = (x_1, x_2, \ldots , x_n)$). We also use the notation $\R^{n}_{>0}:= \braces*{ \boldsymbol{x}^{n} \in \R^{n}: x_i >0, \forall i}$, \mbox{$\R^{n}_{\ge0}:= \braces*{ \boldsymbol{x}^{n} \in \R^{n}: x_i \ge 0, \forall i}$} and $[n] =\{1,2, \ldots , n\}$, for any $n \in \mathbb{N} \backslash \{0\}$. We use the notation $\play$ to denote a player and $-\play$ to indicate her opponent. We also use the standard asymptotic notation $\bigoh$ and its variant $\tilde{\bigoh}$ which ignores logarithmic terms.
% \footnote{Formally, we write $f(\boldsymbol{z}) = \mO\left(g(\boldsymbol{z}) \right)$ (over a set $S \subset \R^{n}_{>0}$) if \mbox{$ \exists M,C >0: |f(\boldsymbol{z})| \le C g(\boldsymbol{z}), \forall \boldsymbol{z} \in S: \boldsymbol{z}_i \ge M, \forall i \in [n]$}.}
Finally, we use $\prob(E)$ to denote the probability of an event $E$ and $\Ex [X] $ to denote the expectation of a random variable~$X$.
	
% The remainder of this paper is organized as follows.
\paragraph {\textbf{Outline of the Paper}}
The remainder of this paper is organized as follows. \cref{sec:Form} introduces the formulations of the {$\FCB$}, \FGL and \FAPA games. We present our complete equilibria characterization of the \FAPA game in \cref{sec:EquiAPA}. Using this result, in \cref{sec:OptUni_GRCBC}, we prove the existence and show the construction of a set of optimal univariate distributions of the $\FCB$ game. In \cref{sec:Corollary_results}, we  derive several corollary results, concerning the equilibria and approximate equilibria of the \FCB and \FGL games, from these optimal univariate distributions. In \cref{sec:heuristic}, we then present an algorithm that efficiently finds an approximation of the proposed optimal univariate distributions with arbitrarily small errors. In \cref{sec:NumExp}, we conduct several numerical experiments illustrating the effect of two types of favoritism in the \FCB and \FGL~games. Finally, we give a concluding discussion in \cref{sec:conclu}.
	
	
	
	
	
	
	
	
	
	
	
	
	
	

==> EC ArXiV - Upload/Sections/num_exp.tex <==


In this section, we conduct numerical experiments illustrating the effect of favoritism in the \FCB and \FGL games. For each game instance, if its parameters satisfy \cref{assum:1} and~\cref{assum:2}, we run the approximation algorithm described in \cref{sec:heuristic} to find a ${\delta}$-approximate solution $\tk = (\tgA, \tgB)$ of the corresponding System~\eqref{eq:system_f} where we set ${\delta} = 10^{-6}$; then, we report the obtained results regarding the distributions $\tAi, \tBi, i \in [n]$ from \cref{def:OptDis_GRCBC} corresponding to~$\tk$. If \cref{assum:1} and~\cref{assum:2} are violated, we report the results corresponding to the trivial pure equilibria. 


	
In the first experiment, we aim to illustrate the relation between parameters $p_i, q_i$ ($i \in [n]$) and the players' equilibrium payoffs in the \FGL game presented in \eqref{eq:payoff_A_GL}-\eqref{eq:payoff_B_GL} (which are also the payoffs of the corresponding \FCB game if the assumptions in \cref{corol:FCBEqui} hold). Since $\FGL$ and $\FCB$ are constant-sum games, we focus on the payoff of Player A. Although our results hold for \FCB and \FGL games in the general setting of parameters, we first focus on instances where the players' budgets are symmetric and all battlefields are homogeneous in order to single out the effect of favoritism. In particular, we consider a group of instances of the \FGL game with $n=4$ battlefields, $X^A = X^B =10$, $\alpha =1/2$, in which all battlefields have the same values ($w_i =1, \forall i$) and the same favoritism parameters $p_i = \bp, q_i = \bq, \forall i$ for given $\bp, \bq$. For comparison, recall that the instance where $\bp= 0, \bq =1$ corresponds to the classical Colonel Blotto/ General Lotto~game.
%
%
%	
 %
	\begin{figure*}[htb!]
		\centering
		\subfloat[$q_1 = q_2 = q_3 = q_4 = \bar{q}$]{
			\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.14\textheight]{Figures/p_runs.png}};
			\node[below=of img, node distance=0cm, yshift=1.1cm, xshift =0.2cm] {\scriptsize$\bp$};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.2cm] {\scriptsize Payoff of Player A};
			\end{tikzpicture}
		}   
				\qquad
		%\subfloat[Expected allocation ]{
		%\begin{tikzpicture}
		%\node (img){\includegraphics[height = 0.14\textheight]{Figures/p_runs_hetero_allo.png}};
	%\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = 0.1cm] {$p$};
	%	\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift = 0cm,yshift = -0.9cm] {\scriptsize Allocation of Player A};
		%\end{tikzpicture}
		%}
		%
		% 		\qquad
		%
			\subfloat[$q_1 = q_2 = \bar{q}$, $q_3 = q_4 = 1/\bar{q}$]{
			\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.14\textheight]{Figures/p_runs_hetero.png}};
			\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = 0.2cm] {\scriptsize$\bp$};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift = 0cm,yshift = -1.0cm] {\scriptsize Payoff of Player A};
			\end{tikzpicture}
		}   
	%
			\caption[]{Equilibrium payoffs of Player A in \FGL games where $n\!=\!4$, $X^A \!=\! X^B = 10$, $\alpha = \frac{1}{2}$; $w_i \!=\! 1$, $p_i\!=\!\bp$,~$\forall i \in [n]$.} \label{fig:Experiment1}
\end{figure*}
%
	
\cref{fig:Experiment1}(a) illustrates the (expected) equilibrium payoff of Player A in instances of the \FGL game where \mbox{$\bp \in \left\{- \! X^A,-\!0.99X^A,\ldots, 0, 0.01{X^A}, 0.02X^A, \ldots, X^A\right\}$} and \mbox{$\bq \in \{{1}/{10}, {1}/{5}, {1}/{2}, 1, 2, 5, 10 \}$}. First we observe that as $\bp$ increases and/or $\bq$ decreases, i.e., favoritism inclines towards Player~A, her expected payoff naturally increases (or at least does not decrease). Second,  most instances satisfy \cref{assum:1} and~\cref{assum:2}; in this case the curves representing Player A's payoffs are piecewise quadratic in $\bp$, which is consistent with its theoretical expression in \eqref{eq:payoff_A_GL}. Third, we observe that the equilibrium payoff of Player A, as a function of $\bp$, is discontinuous at several points. This is due to the fact that for instances where $\bp$ is very small or when $\bq$ is very large (i.e., Player B has strong favoritism), the game has trivial equilibria where Player B can guarantee to win all battlefields (and thus, Player A's payoff is 0). 
% For example, when $q \ge 2$ and $p_i \le -6$, Player B can allocate 2.5 units of resources to each battlefield and guarantees that \mbox{$ q_i \cdot 2.5 - p_i \ge 2\cdot 2.5 + 6 = 11 > X^A$}, thus she wins all battlefields. Reversely, when $\bp$ is large (and/or $\bq$ is~small), there exist trivial equilibria in which Player A can guarantee to win all battlefields and has a payoff of~4. 
	 
Next, we consider game instances with the same $n, X^A, X^B, w_i$ and $p_i$, but we allow resource's effectiveness to vary across battlefields, in particular, $q_1 = q_2 = \bq$ and $q_3 = q_4 = 1/\bq$ where \mbox{$\bq \in \{0.1, 0.2,0.5 \}$}. \cref{fig:Experiment1}(b) reports Player A’s equilibrium payoff in these cases. First, we observe that when $\bp = 0$, the game is symmetric and each player's equilibrium payoff is precisely $ \sum_{i \in [n]} {w_i} /2 = 2$. Contrary to the case of \cref{fig:Experiment1}(a), however, in \cref{fig:Experiment1}(b) when $\bp$ is large, Player A can no longer guarantee to win all battlefields.
% (while the behavior of her payoffs when $\bp$ is very small is similar to that of \cref{fig:Experiment1}(a)).
Moreover, in cases where $\bar{q_i} \in \{0.1, 0.2\}$, when $\bp \ge 2$ and it increases (i.e., Player A has strong pre-allocations), she cannot improve much her payoff. This is explained by the fact that although Player A can guarantee to win battlefields 1 and 2 (where $q_i$ is small), the effectiveness of her resources in battlefields 3 and 4 is too weak so she does not gain much in these battlefields. This illustrates the different effect on equilibrium of the favoritism in resources' effectiveness and in~pre-allocations. 

	 


	


In the next experiment, we consider the following situation: players compete on $n =4$ battlefields where $w_1 = w_2 = w_3 = 1$, $w_4 = 5$ and $q_i = 1, \forall i$ (i.e., resources have the same effectiveness). Player A has a total budget $X^* = 10$, but in this experiment a proportion $P < X^*$ taken out of this budget is pre-allocated. Then, Players A and B play an \FGL (or an \FCB) game where Player A's budget is $X^A = 10 - P$, Player B's budget is $X^B = 10$, and $p_i \ge 0$ such that $\sum_{i \in [n]} p_i = P$. We aim to analyze Player A's payoff when $P$ increases (i.e., when more and more of her budget is committed as pre-allocation).
% and study, for a fixed $P$, how this payoff changes with the distribution of the pre-allocation over the battlefields.
While interesting, we leave the question of what is an optimal distribution of pre-allocation as future work; here we simply compare two simple distributions of Player A's pre-allocation: (i) in the \emph{spread strategy}, the pre-allocation is spread over all battlefields: $p_i = P/n, \forall i \in [n]$; (ii) in the \emph{focus strategy}, the pre-allocation is concentrated on battlefield 4 (the battlefield with a large value): $p_1 = p_2 = p_3 = 0$ and $p_4 = P$.
%
\begin{figure*}[h!]
		\centering
		\subfloat[]{
			\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.20\textwidth]{Figures/XA_split_values.png}};
			\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = 0.1cm] {\scriptsize $P$};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift = 0cm,yshift = -1.0cm] {\scriptsize Payoff of Player A};
			\end{tikzpicture}
		}   
				\quad
		\subfloat[]{
			\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.20\textwidth]{Figures/XA_split_allocate.png}};
			\node[below=of img, node distance=0cm, yshift=1.1cm, xshift = -1.7cm] {\scriptsize $P$};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift = 0cm,yshift = -1.0cm] {\scriptsize Allocations of Player A};
			\end{tikzpicture}
		}   
		% 		\qquad
		%
%
		\caption[]{Player A's equilibrium payoffs and expected allocations in the \FGL game where $n=4$, \mbox{$w_1 = w_2 = w_3 = 1$}, $w_4 = 5$, $X^A = 10 - P$, $X^B = 10$, $q_i = 1, \forall i$ and $\sum_{i \in [n]}{p_i} =P$.} \label{fig:Experiment2}
\end{figure*}
%
	
\cref{fig:Experiment2}(a) illustrates Player A's equilibrium payoff in the \FGL games as described above with $P \in \left\{0,0.1, \ldots, 9.9 \right\}$.  When $P=0$, it is the classical CB game and in this case, the game is symmetric, thus, each player has an equilibrium payoff $\sum_{i \in [n]}w_i /2 =4$. As $P$ increases, Player A's payoff decreases; intuitively, when the proportion of Player A's budget that is pre-allocated increases, she reveals more information about her (pre-)allocations and has less flexibility in play.
% \footnote{Note that as $P = 9.9$, Player B still cannot guarantee to win all battlefields, therefore, Player A's payoff, while small, is still~positive.}
Interestingly, we observe that in instances where $P$ is relatively large, Player A gets a better payoff by distributing the pre-allocations using the focus strategy rather than by the spread strategy, \ie it is better for Player A to focus on ``securing'' the big battlefield. In \cref{fig:Experiment2}(b), we plot the expected allocations of Player A at equilibrium, alone and when added to her pre-allocations (note that since the parameters on battlefields 1, 2, 3 are identical, Player A's expected allocations are the same on these battlefields). As $P$ increases, Player A' expected allocations to the battlefields decrease since her budget \mbox{$X^A = X^* - P$} is reduced (although the aggregate of her allocation and pre-allocation increases in some cases). Interestingly, when $P$ is relatively small, Player A's expected allocations to battlefield 4 is much larger than that at battlefield 1 (this is because $w_4 > w_1$). However, when $P$ increases and under the focus strategy for pre-allocation, her allocation at battlefield 4 decreases quicker than that with the spread strategy. This is consistent with the intuition above that she already ``secures'' this battlefield by the focus strategy thus, she should not distribute a large allocation~there.
%	
%	

	
	
	
	
	
	
	
	
	

	
	
